Bandits with Knapsacks

Multi-armed bandit problems are the predominant theoretical model of exploration-exploitation tradeoffs in learning, and they have countless applications ranging from medical trials, to communication networks, to Web search and advertising. In many of these application domains the learner may be constrained by one or more supply (or budget) limits, in addition to the customary limitation on the time horizon. The literature lacks a general model encompassing these sorts of problems. We introduce such a model, called "bandits with knapsacks", that combines aspects of stochastic integer programming with online learning. A distinctive feature of our problem, in comparison to the existing regret-minimization literature, is that the optimal policy for a given latent distribution may significantly outperform the policy that plays the optimal fixed arm. Consequently, achieving sublinear regret in the bandits-with-knapsacks problem is significantly more challenging than in conventional bandit problems. We present two algorithms whose reward is close to the information-theoretic optimum: one is based on a novel "balanced exploration" paradigm, while the other is a primal-dual algorithm that uses multiplicative updates. Further, we prove that the regret achieved by both algorithms is optimal up to polylogarithmic factors. We illustrate the generality of the problem by presenting applications in a number of different domains including electronic commerce, routing, and scheduling. As one example of a concrete application, we consider the problem of dynamic posted pricing with limited supply and obtain the first algorithm whose regret, with respect to the optimal dynamic policy, is sublinear in the supply.

==> BwK-algorithm.tex <==
\section{[Deprecated!] Two algorithms for \BwK}
\label{sec:algs}

Our main contribution is a pair of algorithms for solving the \BwK problem: a ``balanced exploration'' algorithm (\kMAB) that prioritizes information acquisition, exploring each arm as frequently as possible given current confidence intervals, and a primal-dual algorithm (\pdbwk) that chooses arms to greedily maximize the estimated reward per unit of resource cost.

The regret bounds for the two algorithms coincide up to logarithmic factors for $\nrsc=O(1)$. Beyond that, two algorithms are complementary: while \pdbwk achieves better worst-case dependence on $\nrsc$, \kMAB is better able to take advantage of domain-specific side information to improve its regret guarantee in favorable instances (see Appendix~\ref{app:Balance-wins} for a simple example).

For each algorithm, we prove a regret bound of the form
\begin{align}\label{eq:regret-LPOPT-OPT}
\Rew \geq \LPOPT - f(\LPOPT) \geq \OPT-f(\OPT),
\end{align}
where $\Rew$ is the expected total reward of the algorithm, and $f()$ depends only on parameters $(\budg,\narms,\nrsc)$. The second inequality follows trivially for both algorithms.%
\footnote{This is because
    $g(x) = \max(x-f(x),0)$
is a non-decreasing function of $x$ for $x\geq 0$, and $\LPOPT\geq \OPT$ by Lemma~\ref{lem:lp-relax}.}
As pointed out in the Introduction, the stronger regret bound $f(\LPOPT)$ has an optimal scaling property:  if all budget constraints, including the time horizon, are increased by the factor of $\alpha$, then the regret bound $f(\LPOPT)$ scales as $\sqrt{\alpha}$.


For continuity reasons, we defer the analysis of the
algorithms until later sections of the paper.
Section~\ref{sec:pdbwk-analysis} presents the analysis of \pdbwk, and Section~\ref{analysis-Balance}
presents the analysis of \kMAB.
%% Additionally (and perhaps more importantly) the two algorithms
%% make complementary conceptual contributions to the theory of
%% online learning algorithms.

\subsection{The balanced exploration algorithm (\kMAB)}
\label{sec:Balance}

%In this section we present our first algorithm for \BwK, which we call algorithm \kMAB.

\OMIT{
Intriguingly, the algorithm matches the logarithmic regret bound of $\ucbone$ for stochastic MAB. $\ucbone$ has been successfully applied to a host of stochastic online learning problems and has become an influential algorithm design technique. We believe that \kMAB, like $\ucbone$, is a very general design principle and has the potential to be a meta-algorithm for solving stochastic online learning problems.
}

The design principle behind \kMAB is to explore as much as possible while avoiding obviously suboptimal strategies.  On a high level, the algorithm is very simple. The goal is to converge on an LP-perfect distribution. The time is divided into phases of $|X|$ rounds each. In the beginning of each phase $p$, the algorithm prunes away all distributions $\D$ over arms that with high confidence are not LP-perfect given the observations so far. The remaining distributions over arms are called \emph{potentially perfect}. Throughout the phase, the algorithm chooses among the potentially perfect distributions. Specifically, for each arm $x$, the algorithm chooses a potentially perfect distribution $\Dpx$ which approximately maximizes $\Dpx(x)$, and ``pulls" an arm sampled independently from this distribution. This choice of $\Dpx$ is crucial; we call it the \emph{balancing step}. The algorithm halts as soon as the time horizon is met, or any of the constraints is exhausted. The algorithm's pseudocode is given below.

\newcommand{\TAB}{\hspace{4mm}}
\floatname{algorithm}{Algorithm}
\begin{algorithm}[h]
\myCaption{\kMAB}
%\label{alg:kMAB}
\begin{algorithmic}[1]
%\PARAMETER $\delta \in (0,1)$
%\WHILE{Run phase $t$ till you don't run out of rounds or resource}
\STATE {\bf For} each phase $p=0,1,2,\, \ldots$ {\bf do}
%\STATE \TAB Recompute a ``confidence interval" $I=I_p$ on the latent structure $\mu$
%\STATE \TAB Recompute $\F=\F_p$ according to \eqref{eq:phase-F}.
\STATE \TAB Recompute the set $\F_p$ of potentially perfect distributions $\D$ over arms.
\STATE \TAB Over the next $|X|$ rounds, for each $x\in X$:
\STATE \TAB\TAB pick any distribution $\D=\Dpx\in \F_p$ such that
                    $\D(x) \geq \tfrac12\, \max_{\D'\in \F_p} \D'(x)$.%
%\STATE \TAB\TAB compute distribution $\D_x\in \F$ which maximizes $\D_x(x)$.
\STATE \TAB\TAB choose an arm to ``pull" as an independent sample from $\D$.
\STATE \TAB\TAB {\bf halt} if time horizon is met or one of the resources is exhausted.
\end{algorithmic}
\end{algorithm}

We believe that \kMAB, like $\ucbone$ \citep{bandits-ucb1}, is a very general design principle and has the potential to be a meta-algorithm for solving stochastic online learning problems.

%We prove the following theorem in Section~\ref{sec:Balance}.
\begin{theorem}\label{thm:Balance}
Consider an instance of \BwK with $d$ resources, $m=|X|$ arms, and the smallest budget $B = \min_i B_i$. Algorithm \kMAB achieves regret
\begin{align}\label{eq:Balance-regret}
\LPOPT - \Rew \leq O(\log(\horizon) \log(\horizon / \narms))
\left(
    \sqrt{\nrsc \narms \LPOPT \,} + \LPOPT
        \sqrt{\frac{\nrsc \narms}{\budg}} \;
\right).
\end{align}
Moreover, \eqref{eq:regret-LPOPT-OPT} holds with $f(\LPOPT)$ equal to the right-hand side of \eqref{eq:Balance-regret}.
\end{theorem}

% 7/27/2014: regret bound before deleting the unnecessary terms.
%
%\asedit{\LPOPT} - \Rew \leq O(\log(\horizon) \log(\horizon / \narms))
%\left(
%    \sqrt{\nrsc \narms \asedit{\LPOPT} \,} + \asedit{\LPOPT} \left(
%        \sqrt{\frac{\nrsc \narms}{\budg}} + \frac{\nrsc \narms}{\budg}
%     \right)
%    + \nrsc \narms
%\right).


%% The meaning of $B$ in Theorem~\ref{thm:Balance} is as follows: in each round, at most the $\tfrac{1}{B}$ fraction of each resource is consumed.

Let us fill in the details in the specification of $\kMAB$. In the beginning of each phase $p$, the algorithm recomputes a ``confidence interval" $I_p$ for the latent structure $\mu$, so that (informally) $\mu\in I_p$ with high probability. Then the algorithm determines which distributions $\D$ over arms can potentially be LP-perfect given that $\mu\in I_p$. Specifically, let $\F_p$ be set of all distributions $\D$ that are LP-perfect for some latent structure $\mu'\in I_p$; such distributions are called \emph{potentially perfect} (for phase $p$).

\OMIT{
\begin{align}\label{eq:phase-F}
 \F_p
    = \bigcup_{\mu'\in I_p} \{ \text{distributions } \}
    \argmax_{\D\in \allD} \LP(\D,\mu').
\end{align}
}

It remains to define the confidence intervals $I_p$. For phase $p=0$, the confidence interval $I_0$ is simply $\domain$, the set of all feasible latent structures. For each subsequent phase $p\geq 1$, the confidence interval $I_p$ is defined as follows. For each arm $x$, consider all rounds before phase $p$ in which this arm has been chosen. Let $N_p(x)$ be the number of such rounds, let $\empir{r}_p(x)$ be the time-averaged reward in these rounds, and let $\empir{c}_{p,i}(x)$ be the time-averaged consumption of resource $i$ in these rounds. We use these averages to estimate $r(x,\mu)$ and $c_i(x,\mu)$ as follows:
\begin{align}
|r(x,\mu) - \empir{r}_p(x)|
    &\leq \rad\left(\, \empir{r}_p(x), N_p(x) \,\right)
    \label{eq:algo-estimate-r}\\
|c_i(x,\mu) - \empir{c}_{p,i}(x)|
    &\leq \rad\left(\, \empir{c}_{p,i}(x), N_p(x) \,\right)
    \quad \text{for each resource $i$}
    \label{eq:algo-estimate-c}
\end{align}
The confidence interval $I_p$ is the set of all latent structures $\mu'\in I_{p-1}$ that are consistent with these estimates. This completes the specification of \kMAB.

For each phase of \kMAB, the round in which an arm is sampled from distribution $\Dpx$ will be called \emph{designated} to arm $x$. We need to use approximate maximization to choose $\Dpx$, rather than exact maximization, because an exact maximizer
    $\argmax_{\D\in \F_p} \D(x)$
is not guaranteed to exist.





==> BwK-analysis.tex <==
\section{Analysis}
\begin{claim}[Properties of the confidence radius]~
\label{cl:conf-rad-props}
\begin{OneLiners}
\item[(a)] monotonicity: $\rad(\nu,N)$ is non-decreasing in $\nu$ and non-increasing in $N$.
\item[(b)] concavity: $\rad(\nu,N)$ is concave in $\nu$, for any fixed $N$.
\item[(c)] $\nu - \rad(\nu,N)$ is non-decreasing in $\nu$.
\item[(d)] $\nu- \rad(\nu,N) \geq \tfrac14\, \nu$ whenever $4\tfrac{\chernoffC}{N} \leq \nu \leq 1$.
\item[(e)] $\rad(\nu,N) \leq 3 \tfrac{\chernoffC}{N}$ whenever $\nu\leq 4\tfrac{\chernoffC}{N}$.
\item[(f)] $\rad(\nu,\alpha N) = \tfrac{1}{\alpha}\, \rad(\alpha\nu,\, N)$,
    for any $\alpha\in (0,1]$.
    \textcolor{red}{\bf A.S.: this property seems very useful.}
\item[(g)]
    $\frac{1}{N}\sum_{\ell=1}^{N} \rad(\nu, \ell) \leq O(\rad(\nu,N))$.
\end{OneLiners}
\end{claim}

\begin{claim}
\label{cl:LP-properties}
Let $\mu$ be some latent distribution over $\outcomes$ and let $\D\in \F(\mu)$. Then the following two properties hold
\begin{OneLiners}
\item[(a)] $c(\D,\mu)=B/T$
\item[(b)] $\D$ has a support of size at most $2$.
\end{OneLiners}
\end{claim}

\begin{proof}
\end{proof}

\begin{claim}
\label{claim:bounderror-Alex}
Fix a phase $t$ in a clean execution of $\A$. Let $\mu',\mu''\in I_t$, and let $\D\in \F_t$. Then
\begin{align}
 | c(\D, \mu') - c(\D, \mu'')|
    &\leq 8\; \rad\left( c(\D,\mu'), t \right).
        \label{eq:claim:bounderror-Alex-c}\\
 | r(\D, \mu') - r(\D, \mu'')|
    &\leq 8\; \rad\left( r(\D,\mu'), t \right).
        \label{eq:claim:bounderror-Alex-r}
\end{align}
\end{claim}


\begin{proof}
We prove \eqref{eq:claim:bounderror-Alex-c}; \eqref{eq:claim:bounderror-Alex-r} is proved similarly.
Let us first prove the following:
\begin{align}\label{eq:inter:errorbound-Alex}
\forall x\in S,\quad
\D(x)\, | c(x,\mu'_x) - c(x,\mu''_x) |\leq
    8\; \rad(\D(x)\, c(x,\mu'_x),t).
\end{align}
From \eqref{eq:high-prob-events-meta} of clean execution we get a lower bound on $N_t(x)$
\begin{align*}
N_t(x)/t \geq n_t(x)/t = \empirdtx{t}{x}
    \geq  \avedtx{t}{x} - \rad(\avedtx{t}{x}, t)
    \geq  \D(x) - \rad(\D(x), t).
\end{align*}
Consider two cases: for the first case, assume
    $\D(x) \geq 4 \tfrac{\chernoffC}{t} $.
Using Claim~\ref{cl:conf-rad-props}(d) and the previous equation, it follows that
    $N_t(x) \geq \tfrac{1}{4}\, t\,\D(x)$.
Therefore:
\begin{align*}
\D(x)\; |c(x,\mu'_x)-c(x,\mu''_x)|
&\leq \D(x)\, \rad(c(x,\mu'_x),\,N_t(x) )
    & \text{(by clean execution)}\\
&\leq \D(x)\, \rad(c(x,\mu'_x),\,\tfrac{1}{4}\, t\,\D(x) )
    & \text{(by monotonicity of $\rad$)}\\
&= 4\, \rad(\D(x)\, c(x,\mu_x'), t)
    & \text{(by Claim~\ref{cl:conf-rad-props}(f))}.
\end{align*}
The second case is that
    $\D(x) < 4 \tfrac{\chernoffC}{t} $.
Then~\eqref{eq:inter:errorbound-Alex} follows simply because
    $\tfrac{\chernoffC}{t} \leq \rad(\cdot\,, t)$.

We complete the proof of \eqref{eq:claim:bounderror-Alex-c} using concavity of $\rad(\cdot, t)$.
\begin{align*}
| c(\D, \mu') - c(\D, \mu'')|
    & \leq \textstyle \sum_{x\in X} \D(x)\, | c(x,\mu'_x) - c(x,\mu''_x) | \\
    &\leq  \textstyle \sum_{x\in X} 4\; \rad(\D(x)\, c(x,\mu'_x),t) \\
    &\leq 8\; \rad\left( \tfrac{1}{2} \,\textstyle \sum_{x\in X} \D(x)\, c(x,\mu'),\; t \right)\\
    &= 8\; \rad\left( \tfrac{1}{2} \, c(\D,\mu'),\; t \right).\qedhere
\end{align*}
(Note that we are using a slightly weaker version, without the $\tfrac{1}{2}$ term.)
\end{proof}

\begin{claim}
\label{cl:distr-ratios-Alex}
Consider the setting in Claim~\ref{claim:bounderror-Alex}. Assume
    $t \geq \gamma^2$,
where
    $\gamma = 16\,\Gamma$.
Then for each resource $i$
$$\left| \frac{r(\D,\mu')}{c(\D,\mu')} - \frac{r(\D,\mu'')}{c(\D,\mu'')} \right|
\leq \gamma\, \rad( 1,\, \nu\,t),
\text{ where }
\nu = \tfrac12\,\max( c(\D,\mu'),\, c(\D,\mu'') ).
$$
\end{claim}

\begin{proof}
Using Claim~\ref{claim:userfulequation1} and \eqref{eq:no-free-lunch-implication},
we obtain:
\begin{align}
\frac{r(\D,\mu')}{c(\D,\mu')} - \frac{r(\D,\mu'')}{c(\D,\mu'')}
    &\leq \frac{|r(\D,\mu') - r(\D,\mu'')|}{c(\D,\mu')}
        + \frac{r(\D,\mu')}{c(\D,\mu')} \; 
        \frac{|c(\D,\mu') - c(\D,\mu'')|}{c(\D,\mu')}  \nonumber \\
    &\leq 8\; \frac{\rad( r(\D,\mu'),\, t) + \Gamma\;\rad( c(\D,\mu'),\, t)}{c(\D,\mu')} \nonumber \\
    &\leq \gamma\; \frac{\rad( c(\D,\mu'),\, t)}{c(\D,\mu')}
        \label{eq:cl:distr-ratios-Alex-1} \\
    &\leq \gamma\; \rad( 1,\, t\,c(\D,\mu')).
        \label{eq:cl:distr-ratios-Alex-2}
\end{align}
To prove \eqref{eq:cl:distr-ratios-Alex-1}, we used the fact that $r(\D,\mu') \leq \Gamma\; c(\D,\mu')$. Note that \eqref{eq:cl:distr-ratios-Alex-2} does not require the assumption that $t\geq \gamma^2$.

Using \eqref{eq:cl:distr-ratios-Alex-1} for the special case $r(\D,\mu') = r(\D,\mu'')$, we find that
$$ c(\D,\mu')
    \geq c(\D,\mu'') (1-\gamma\, \rad( c(\D,\mu'),\, t))
    \geq c(\D,\mu'') (1-\gamma/\sqrt{t})
    \geq \tfrac12\, c(\D,\mu'').
$$
We complete the proof using \eqref{eq:cl:distr-ratios-Alex-1} with the roles of $\mu'$ and $\mu''$ reversed.
\end{proof}

\begin{claim}
\label{cl:lpconvergence-Alex}
Consider the setting in Claim~\ref{claim:bounderror-Alex}. Assume
    $t \geq \gamma^2$,
where
    $\gamma = 16\,\Gamma$.
Then
$$ \LP(\D,\mu')- \LP(\D,\mu'')\leq 4\gamma\; T\; \rad\left( B/T,\; t \right).
$$
\end{claim}

\begin{proof}
Since $\D\in \F_t$ we know that for some $\mu\in I_t$ we have that $\D\in \F(\mu)$. Then from claim \ref{cl:LP-properties} we have that $c(\D,\mu)=B/T$.
We have:
\begin{align*}
\LP(\D,\mu')- \LP(\D,\mu)
    &\leq  \frac{B\, r(\D,\mu')}{c(\D,\mu')} - \frac{B\, r(\D,\mu)}{c(\D,\mu)}
        & \\
    &\leq 2\gamma\, B\; \rad(1, t\, c(\D,\mu))
        & \text{by Claim~\ref{cl:distr-ratios-Alex}} \\
    &\leq 2\gamma\, B\; \rad(1, t\, B/T)
        & \text{used tightness of $j$} \\
    &\leq 2\gamma\, T\; \rad(B/T, t)
         & \text{by Claim~\ref{cl:conf-rad-props}(f)}. \qquad\qedhere
\end{align*}
We can similarly show that $ \LP(\D,\mu)- \LP(\D,\mu'')\leq 2\gamma\; T\; \rad\left( B/T,\; t \right)$. Adding the two equations we get $ \LP(\D,\mu')- \LP(\D,\mu'')\leq 4\gamma\; T\; \rad\left( B/T,\; t \right)$.
\end{proof}


\begin{claim}
\label{cl:LP-of-Dt}
Fix a phase $t$ in a clean execution of $\A$ and let $\D\in \F_t$. Assume
    $t \geq \gamma^2$,
where
    $\gamma = 16\,\Gamma$. Then for any $\mu'\in I_t$ we have
$$\LP(\D^*,\mu^*) - \LP(\D_t,\mu^*)
    \leq  4\gamma\; T\; \rad\left(B/T,\; t \right).
$$
\end{claim}

\begin{proof}
Recall that $\D_t, \D^* \in \F_t$. In words, $\D_t$ maximizes $\LP(\D,\mu'')$ for some latent structure $\mu''\in I_t$, and $\D^*$ maximizes $\LP(\D,\mu^*)$ for some latent structure $\mu^*$. We can apply Lemma~\ref{cl:lpconvergence-Alex} with $\D = \D_t$ and $\D = \D^*$.

For brevity, denote
    $\Phi  = \gamma\; T\; \rad\left(B/T,\; t \right)$.
Then we get
\begin{align*}
\LP(\D_t,\mu^*)
    &\geq \LP(\D_t,\mu'')- 2 \Phi
    &\textrm{by Lemma~\ref{cl:lpconvergence-Alex}} &\\
    &\geq\LP(\D^*,\mu'')- 2\Phi \\
    &\geq \LP(\D^*,\mu^*)-
        4\Phi
         &\textrm{by Lemma~\ref{cl:lpconvergence-Alex}} &\qedhere
\end{align*}
\end{proof}



\begin{claim}
\label{cl:BasicBwK-LP-of-Dt}
Fix round $t$. Assume
    $t \geq \gamma^2$,
where
    $\gamma = 32\,\Gamma$. Then
$$\LP(\D_t,\mu) \geq \LPOPT
    -  4\gamma\; T\; \rad\left( \tfbt,\; t \right).
$$
\end{claim}

\begin{corollary}
\label{cor:BasicBwK-Rew}
For each phase $t$
$$\Rew_t \geq \frac{t\, |X|}{T}\; \LPOPT
    -  O(\Gamma\, t\, |X|)\; \rad\left( \frac{B+\LPOPT}{T},\; t \right) - O(\Gamma^2\, |X|).
$$
\end{corollary}

\begin{proof}
Assume
    $t \geq \gamma^2$,
where
    $\gamma = 32\,\Gamma$.
By Claim~\ref{cl:BasicBwK-LP-of-Dt},
$$ r(\D_t,\mu) \geq \tfrac{1}{T} \LP(\D_t,\mu)
    \geq \tfrac{1}{T}\, \LPOPT - 4\gamma\, \rad(\tfbt, t).
$$
Averaging the above equation over all rounds (excluding the first $\gamma^2$ such phases), and using Claim~\ref{cl:conf-rad-props}(g) to average the confidence radii, we have:
\begin{align*}
r(\aveD_t,\mu)
    \geq \tfrac{1}{T} \LPOPT -  O(\gamma)\, \rad(\tfbt, t) -\gamma^2/t.
\end{align*}
Using the corresponding high-probability event in~\eqref{eq:high-prob-events-meta}:
$$ \frac{\Rew_t}{t\, |X|}
    = r(\empir{\D}_t, \empir{\mu}_t)
    \geq r(\aveD,\mu) - \rad( r(\aveD,\mu), t ).
$$
Now using the monotonicity of $\nu - \rad(\nu,N)$ we obtain
\begin{align*}
 \frac{\Rew_t}{t\, |X|}
    &\geq \tfrac{1}{T} \LPOPT -  4\gamma\, \rad(\tfbt, t) -\gamma^2/t
        - \rad(\tfrac{1}{T} \LPOPT,\; t). \qedhere
\end{align*}
\end{proof}


\begin{claim}
\label{cl:BasicBwK-supply}
For each phase $t$ we have
$ c(\D_t, \mu) \leq \tfbt + 16\,\rad\left(\tfbt,\; t \right). $
\end{claim}

\begin{proof}
Take $\mu'$ such that $\D_t \in \F(\mu')$. Apply Claim~\ref{claim:bounderror-Alex}, noting that $c_t(\D_t,\mu') = \fbt$ (by Claim~\ref{cl:LP-properties}).
\end{proof}

Let $B_t$ be the supply utilization at time $t$.

\begin{corollary} \label{cor:BasicBwK-supply}
    $\frac{B_t}{t\, |X|} \leq \tfbt + O(\rad(\tfbt, t)) $.
\end{corollary}
\begin{proof}
Using the corresponding high-probability event in~\eqref{eq:high-prob-events-meta}:
$$ \frac{B_t}{t\, |X|} = c(\empir{D}_t, \empir{\mu}_t)
    \leq c(\aveD, \mu) + \rad\left( c(\aveD, \mu),\; t\right).
$$
Averaging Claim~\ref{cl:BasicBwK-supply} over all rounds when the meta-arm $S$ was chosen, and using Claim~\ref{cl:conf-rad-props}(g) to average the confidence radii, we have:
$$ c(\aveD, \mu) \leq \tfbt + O(\rad(\tfbt, t)).
$$
Using the property of the confidence radius that
$$ \rad(\rad(\nu,N),\,N) \leq O(\rad(\nu,N)),
$$
we conclude that
$ \rad\left( c(\aveD, \mu),\; t\right) \leq O(\rad(\tfbt, t)),
$
and the claim follows.
\end{proof}

\begin{theorem}\label{lm:basicBwK-totalrevenue}
Let $\alpha = 1+\LPOPT/B$. Then the algorithm has total revenue
\begin{align}\label{eq-lm:basicBwK-totalrevenue}
%\Rew \geq \LPOPT - O(\alpha\,\Gamma T)\; \rad(\alpha\,\tfbt,\; T/|X|) - O(\Gamma^2).
\Rew \geq \LPOPT - O(\alpha\, \Gamma\, \chernoffC(\sqrt{B |X|}+|X|)) - O(\Gamma^2).
\end{align}
\end{theorem}

\begin{proof}
The algorithm stops either when it runs out of time or if it runs out of resource. To bound the total revenue let us first get a bound on the stopping time of the algorithm. If the algorithm stops at time $t$ because it runs out of time then trivially $t=T/|X|$. Otherwise if it runs out of resource then $B_t\geq B$. If we substitute this in Corollary \ref{cor:BasicBwK-supply} we get the following lower bound on $t$
$$ \tfrac{t\, |X|}{T}
    \geq 1 - O(\tfrac{t\, |X|}{B})\; \rad(\tfbt,\, t).
$$
Substituting this back in Corollary \ref{cor:BasicBwK-Rew} we a bound on the total revenue
\begin{align}\label{eq-lm:basicBwK-interface-1}
\Rew_t \geq& \LPOPT
    - O(\alpha\,\Gamma t\, |X|)\; \rad(\alpha\,\tfbt,\; t) - O(\Gamma^2) \\
\geq& \LPOPT - O(\alpha\,\Gamma T)\; \rad(\alpha\,\tfbt,\; T/|X|) - O(\Gamma^2) \\
\geq& \LPOPT - O(\alpha\, \Gamma\, \chernoffC(\sqrt{B |X|}+|X|)) - O(\Gamma^2)
\end{align}
\end{proof}


==> BwK-multiAnalysis.tex <==
\section{[Deprecated!] Analysis of \kMAB (proof of Theorem~\ref{thm:Balance})}
\label{analysis-Balance}

Let us summarize various properties of the confidence radius which we use throughout the analysis.

\begin{claim}
\label{cl:conf-rad-props}
The confidence radius $\rad(\nu,N)$, defined in \eqref{eq:conf-rad-defn}, satisfies the following properties:
\begin{OneLiners}
\item[(a)] monotonicity: $\rad(\nu,N)$ is non-decreasing in $\nu$ and non-increasing in $N$.
\item[(b)] concavity: $\rad(\nu,N)$ is concave in $\nu$, for any fixed $N$.
\item[(c)] $\max(0,\; \nu - \rad(\nu,N))$ is non-decreasing in $\nu$.
\item[(d)] $\nu- \rad(\nu,N) \geq \tfrac14\, \nu$ whenever $4\tfrac{\chernoffC}{N} \leq \nu \leq 1$.
\item[(e)] $\rad(\nu,N) \leq 3 \tfrac{\chernoffC}{N}$ whenever $\nu\leq 4\tfrac{\chernoffC}{N}$.
\item[(f)] $\rad(\nu,\alpha N) = \tfrac{1}{\alpha}\, \rad(\alpha\nu,\, N)$,
    for any $\alpha\in (0,1]$.
\item[(g)]
    $\frac{1}{N}\sum_{\ell=1}^{N} \rad(\nu, \ell)
        \leq O(\log N)\;\rad(\nu,N)$.
\end{OneLiners}
\end{claim}

\subsection{Deterministic properties of \kMAB}

First, we show that any two latent structures in the confidence interval $I_p$ correspond to similar consumptions and rewards, for each arm $x$. This follows deterministically from the specification of $I_p$.

\begin{claim}
\label{cl:bdd-error-x}
Fix any phase $p$, any two latent structures $\mu',\mu''\in I_p$, an arm $x$, and a resource $i$. Then
\begin{align}
\ | c_i(x, \mu') - c_i(x, \mu'')|&\leq 6\; \rad\left( c_i(x,\mu'), N_p(x) \right) \label{eq:cl:bdd-error-x-c}\\
 | r(x, \mu') - r(x, \mu'')|&\leq 6\; \rad\left( r(x,\mu'), N_p(x) \right).\label{eq:cl:bdd-error-x-r}
\end{align}
\end{claim}
\begin{proof}
We prove \eqref{eq:cl:bdd-error-x-c}; \eqref{eq:cl:bdd-error-x-r} is proved similarly.

Let $N = N_p(x)$.
%    $\Phi(\mu') = \rad\left( c_i(x,\mu'), N_p(x) \right)$.
By specification of \kMAB, any $\mu'\in I_p$ is consistent with estimate~\refeq{eq:algo-estimate-c}:
$$|c_i(x,\mu') - \empir{c}_{p,i}(x)|
    \leq \rad\left(\, \empir{c}_{p,i}(x), N \,\right).
$$
It follows that
$$ | c_i(x, \mu') - c_i(x, \mu'')| \leq 2\; \rad\left( \empir{c}_{p,i}(x), N \right).
$$
Finally, we observe that by Claim~\ref{cl:rad-to-rad},
$$\rad\left( \empir{c}_{p,i}(x), N \right) \leq 3\,\rad\left( c_i(x,\mu'), N \right).
\qedhere
$$
\end{proof}

For each phase $p$ and arm $x$, let
    $\avedtx{p}{x}=\frac{1}{p}\sum_{q< p}\Dqx(x)$
be the average of probabilities for arm $x$ among the distributions in the preceding phases that are designated to arm $x$. Because of the balancing step in \kMAB, we can compare this quantity to $\D(x)$, for any $\D\in \F_p$. (Here we also use the fact that the confidence intervals $I_p$ are non-increasing from one phase to another.)

\begin{claim}
\label{cl:Dpx}
$\avedtx{p}{x}\geq \tfrac12\,\D(x)$
for each phase $p$, each arm $x$ and any distribution $\D\in \F_p$.
\end{claim}
\begin{proof}
Fix arm $x$. Recall that
    $\avedtx{p}{x}=\frac{1}{p}\sum_{q< p}\Dqx(x)$,
where $\Dqx$ is the distribution chosen in the round in phase $q$ that is designated to arm $x$. Fix any phase $q<p$. Because of the balancing step, $\Dqx(x) \geq \tfrac12\, \D'(x)$ for any distribution $\D'\in \F_q$. Since the confidence intervals $I_q$ are non-increasing from one phase to another, we have $I_p\subset I_q$ for any $q\leq p$, which implies that $\F_p \subset \F_q$. Consequently, $\Dqx(x) \geq \tfrac12\, \D(x)$ for each $q< p$, and the claim follows.
\end{proof}

\subsection{High-probability events}


We keep track of several quantities: the averages $\empir{r}_p(x)$ and $\empir{c}_{p,i}(x)$ defined in Section~\ref{sec:Balance}, as well as several other quantities that we define below.

Fix phase $p$. For each arm $x$, consider all rounds in phases $q <p$ that are designated to arm $x$. Let $n_p(x)$ denote the number of times arm $x$ has been chosen in these rounds.
Let $\empirdtx{p}{x}=n_t(x)/p$ be the corresponding empirical probability of choosing $x$. We compare this to $\avedtx{p}{x}$.

\OMIT{Let
    $\avedtx{p}{x}=\frac{1}{p}\sum_{q< p}\Dqx(x)$
be the average of probabilities for arm $x$ among the distributions chosen for these rounds.}

Further, consider all rounds in phases $q< p$. There are $N = p|X|$ such rounds. The average distribution chosen by the algorithm in these rounds is
    $\aveD_p = \tfrac{1}{N} \sum_{q< p,\, x\in X} \Dqx $.
We are interested in the corresponding quantities
    $r(\aveD_p, \mu)$ and $c_i(\aveD_p, \mu)$,
We compare these quantities to
    $\empir{r}_p = \tfrac{1}{N} \sum_{t=1}^N r_t$
and
    $\empir{c}_{p,i} = \tfrac{1}{N} \sum_{t=1}^N c_{t,i}$,
the average reward and the average resource-$i$ consumption in phases $q<p$.

We consider several high-probability events which follow from applying Theorem~\ref{thm:conf-rad} to the various quantities defined above. All these events have a common shape: $\empir{\nu}$ is an $N$-strong estimate for $\nu$, for some quantities $\nu,\empir{\nu}\in[0,1]$ and $N\in \N$.

\begin{lemma}\label{lm:high-prob-events}
For each phase $p$, arm $x$, and resource $i$, with probability $e^{-\Omega(\chernoffC)}$ it holds that:
\begin{itemize}
\item[(a)] $\empir{r}_p(x)$ is an $N_p(x)$-strong estimator for $r(x,\mu)$, and
$\empir{c}_{p,i}(x)$ is an $N_p(x)$-strong estimator for $c_i(x,\mu)$.

\item[(b)] $\avedtx{p}{x}$ is an $p$-strong estimator for $\empirdtx{p}{x}$.

\item[(c)] $r(\aveD_p,\, \mu)$  is an $(p|X|)$-strong estimator for $\empir{r}_p$,
and $c_i(\aveD_p,\, \mu)$ is an $(p|X|)$-strong estimator for
 $\empir{c}_{p,i}$.
\end{itemize}
\end{lemma}


\subsection{Clean execution of \kMAB}

A \emph{clean execution} of the algorithm is one in which all events in Lemma~\ref{lm:high-prob-events} hold. It is convenient to focus on a clean execution.
In the rest of the analysis, we assume clean execution without further notice. Also, we fix an arbitrary phase $p$ in such execution.

% In the rest of the analysis, we focus on a clean execution.

Since a clean execution satisfies the event in Claim~\ref{lm:high-prob-events}(a), it immediately follows that:

\begin{claim}
The confidence interval $I_p$ contains the (actual) latent structure $\mu$. Therefore, $\D^*\in \F_p$ for any distribution $\D^*$ that is LP-perfect for $\mu$.
\end{claim}



\begin{claim}
\label{claim:bounderror-Alex}
Fix any latent structures $\mu',\mu''\in I_p$ and any distribution $\D\in \F_p$. Then for each resource $i$,
\begin{align}
 %\|C(\mu')\D-C(\mu'')\D\|_{\infty}&\leq\; \sqrt{\frac{B}{tT}} \label{eq:claim:bounderror-Alex-c}\\
 | c_i(\D, \mu') - c_i(\D, \mu'')|&\leq O(1)\; \rad\left( c_i(\D,\mu'),\, p/d \right) \label{eq:claim:bounderror-Alex-c}\\
 | r(\D, \mu') - r(\D, \mu'')|&\leq O(1)\; \rad\left( r(\D,\mu'),\, p/d \right).\label{eq:claim:bounderror-Alex-r}
\end{align}
\end{claim}

\begin{proof}
We prove \eqref{eq:claim:bounderror-Alex-c}; \eqref{eq:claim:bounderror-Alex-r} is proved similarly.
Let us first prove the following:
\begin{align}\label{eq:inter:errorbound-Alex}
\forall x\in X,\quad
\D(x)\, | c_i(x,\mu') - c_i(x,\mu'') |\leq
    O(1)\; \rad(\D(x)\, c_i(x,\mu'),p).
\end{align}
Intuitively, in order to argue that we have good estimates on quantities related to arm $x$, it helps to prove that this arm has been chosen sufficiently often. Using the definition of clean execution and Claim~\ref{cl:Dpx}, we accomplish this as follows:
\begin{align*}
\tfrac{1}{p}\, N_p(x)
    &\geq \tfrac{1}{p}\, n_p(x)
    = \empirdtx{p}{x} \\
    &\geq  \avedtx{p}{x} - \rad(\avedtx{p}{x}, p) & \text{(by clean execution)} \\
    &\geq  \tfrac12\,\D(x) - \rad(\tfrac12\,\D(x), p)
        & \text{(by Claim~\ref{cl:Dpx} and Claim~\ref{cl:conf-rad-props}(c))}.
\end{align*}
Consider two cases depending on $\D(x)$. For the first case, assume
    $\D(x) \geq 8 \tfrac{\chernoffC}{p} $.
Using Claim~\ref{cl:conf-rad-props}(d) and the previous equation, it follows that
    $N_p(x) \geq \tfrac{1}{8}\, p\,\D(x)$.
Therefore:
\begin{align*}
\D(x)\; |c_i(x,\mu')-c_i(x,\mu'')|
&\leq 6\;\D(x)\, \rad(c_i(x,\mu'),\,N_p(x) )
    & \text{(by Claim~\ref{cl:bdd-error-x})}\\
&\leq 6\;\D(x)\, \rad(c_i(x,\mu'),\,\tfrac{1}{8}\, p\,\D(x) )
    & \text{(by monotonicity of $\rad$)}\\
&= 48\; \rad(\D(x)\, c_i(x,\mu_x'), p)
    & \text{(by Claim~\ref{cl:conf-rad-props}(f))}.
\end{align*}
The second case is that
    $\D(x) < 8 \tfrac{\chernoffC}{p} $.
Then \eqref{eq:inter:errorbound-Alex} follows simply because
    $\tfrac{\chernoffC}{p} \leq \rad(\cdot\,, p)$.

We have proved \eqref{eq:inter:errorbound-Alex}. We complete the proof of \eqref{eq:claim:bounderror-Alex-c} using concavity of $\rad(\cdot, p)$ and the fact that, by the specification of \kMAB, $\D$ has support of size at most $d$.
\begin{align*}
| c_i(\D, \mu') - c_i(\D, \mu'')|
    & \leq \textstyle \sum_{x\in X} \D(x)\, | c_i(x,\mu') - c_i(x,\mu'') | \\
    &\leq  \textstyle \sum_{x\in X,\D(x)>0} O(1)\; \rad(\D(x)\, c_i(x,\mu'),p) \\
    &\leq O(d)\; \rad\left( \tfrac{1}{d} \,\textstyle \sum_{x\in X} \D(x)\, c_i(x,\mu'),\; p \right)\\
    &= O(d)\; \rad\left( \tfrac{1}{d} \; c_i(\D,\mu'),\; p \right) \\
    &\leq O(1)\; \rad\left( c_i(\D,\mu'),\; \tfrac{p}{d} \right)
        \qquad \text{(by Claim~\ref{cl:conf-rad-props}(f))}. \qedhere
\end{align*}
\end{proof}


In what follows, we will denote
    $\ucblp_p    = \max_{\D\in \F_p,\;\mu\in I_p}\LP(\D,\mu)$.

\begin{claim}
\label{cl:lpconvergence-Alex}
Fix any latent structures $\mu',\mu''\in I_p$ and any distribution $\D\in \F_p$. Then
\begin{align}\label{eq:cl:lpconvergence-Alex}
|\LP(\D,\mu')-\LP(\D,\mu'')|
    &\leq O(T)\, \rad\left( \ucblp_p/T,\; \tfrac{p}{d} \right)
        + O(\ucblp_p\, \tfrac{T}{B})\,\rad\left(\tfbt,\tfrac{p}{d}\right).
%    &\leq \abedit{\Phi_p(\ucblp_p)}.
\end{align}
\end{claim}

\begin{proof}
Since $\D\in \F_p$, it is LP-perfect for some latent structure $\mu$. Then
    $\LP(\D,\mu) = T\, r(\D,\mu)$.
Therefore:
\begin{align}
\LP(\D,\mu')-\LP(\D,\mu)
&\leq\;T\,\left( r(\D,\mu')- r(\D,\mu) \right) & \nonumber \\
&\leq\;O(T)\;\rad\left( r(\D,\mu), \tfrac{p}{d} \right)
    & \text{(by Claim~\ref{claim:bounderror-Alex})}.
        \label{eq:cl:lpconvergence-Alex-easy}
\end{align}

We need a little more work to bound the difference in the $\LP$ values in the other direction.

Consider
    $t_0 = \LP(\D,\mu')/  r(\D,\mu')$;
this is the value of the variable t in the optimal solution to the linear program~\refeq{eq:LP-D}. Let us obtain a lower bound on this quantity. Assume $t_0<T$. Then one of the budget constraints in~\refeq{eq:LP-D} must be tight, i.e. $t_0\, c_i(\D,\mu') = B$ for some resource $i$.
\begin{align*}
c_i(\D,\mu')
    &\leq c_i(\D,\mu)+O(1)\,\rad\left(c_i(\D,\mu),\tfrac{p}{d} \right)
        & \text{(by Claim~\ref{claim:bounderror-Alex})} \\
    &\leq \tfbt+O(1)\,\rad\left(\tfbt,\tfrac{p}{d}\right)
\end{align*}
Let $\Psi = \rad\left(\tfbt,\tfrac{p}{d}\right) $.
It follows that
    $t_0 = B/c_i(\D,\mu')  \geq T(1- O(\tfrac{T}{B}\,\Psi)).$
Therefore:
\begin{align*}
\LP(\D,\mu)-\LP(\D,\mu')
    &=\;T\, r(\D,\mu)-t_0\,r(\D,\mu') \\
    &\leq T\,r(\D,\mu)- \left[ T(1- O(\tfrac{T}{B}\,\Psi)) \right] \;  r(\D,\mu') \\
    &\leq T\, \left[ r(\D,\mu)- r(\D,\mu') \right]
        + O(\tfrac{T}{B}\,\Psi) \,T\, r(\D,\mu)  \\
    &\leq O(T)\, \rad\left( r(\D,\mu), \tfrac{p}{d} \right)
        + O(\tfrac{T}{B}\,\Psi)\,T\, r(\D,\mu)
    & \text{(by Claim~\ref{claim:bounderror-Alex})}.
\end{align*}
Using \eqref{eq:cl:lpconvergence-Alex-easy} and noting that
    $r(\D,\mu) = \LP(\D,\mu) / T \leq \ucblp_p/T$,
we conclude that
\begin{align*}
|\LP(\D,\mu)-\LP(\D,\mu')|
    &\leq O(T)\, \rad\left( \ucblp_p/T,\; \tfrac{p}{d} \right)
        + O(\ucblp_p\, \tfrac{T}{B})\,\rad\left(\tfbt,\tfrac{p}{d}\right).
\end{align*}
We obtain the same upper bound on
    $|\LP(\D,\mu)-\LP(\D,\mu'')|$,
and the claim follows.
\end{proof}

We will use $\Phi_p(\ucblp_p)$ to denote the right-hand side of \eqref{eq:cl:lpconvergence-Alex}.

\begin{claim}
\label{cl:LP-of-Dt}
~%\abedit{Let $\Phi_p=\Phi_p(\LPOPT)$}
\begin{itemize}
\item[(a)]
Fix any latent structure $\mu^*\in I_p$, and any distributions $\D',\D''\in \F_p$.
Then
$$|\LP(\D',\mu^*) - \LP(\D'',\mu^*)|\leq 2 \Phi_p(\ucblp_p)$$
\item[(b)]
Fix any latent structure $\mu',\mu''\in I_p$, and any distributions $\D',\D''\in \F_p$.
Then
$$|\LP(\D',\mu') - \LP(\D'',\mu'')|\leq 3 \Phi_p(\ucblp_p)$$
\end{itemize}
\end{claim}

\begin{proof}
{\bf (a).} Since $\D',\D''\in \F_p$, it holds that $\D'$ and $\D''$ are LP-perfect for some latent structures $\mu'$ and $\mu''$. Further, pick a distribution $\D^*$ that is LP-perfect for $\mu^*$. Then:
\begin{align*}
\LP(\D',\mu^*)
    &\geq \LP(\D',\mu')- \Phi_p(\ucblp_p)
    &\textrm{(by Lemma~\ref{cl:lpconvergence-Alex} with $\D = \D'$)} &\\
    &\geq\LP(\D^*,\mu')- \Phi_p(\ucblp_p) \\
    &\geq \LP(\D^*,\mu^*)- 2\Phi_p(\ucblp_p)
    &\textrm{(by Lemma~\ref{cl:lpconvergence-Alex} with $\D =\D^*$)} &\\
    &\geq \LP(\D'',\mu^*)- 2\Phi_p(\ucblp_p). &&
\end{align*}

{\bf (b).} Follows easily from part (a) and Lemma~\ref{cl:lpconvergence-Alex}. \qedhere
\end{proof}

The following claim will allow us to replace $\Phi_p(\ucblp_p)$ by $\Phi_p(\LPOPT)$.%
\footnote{$\Phi_p(\LPOPT)$ is the right-hand side of \eqref{eq:cl:lpconvergence-Alex} with $\LPOPT$ instead of $\ucblp_p$.}

\begin{claim}\label{cl:LP-phip-substitute}
$\Phi_p(\LPOPT)\geq \Omega(\max(\LPOPT,\Phi_p(\ucblp_p)))$.
\end{claim}
\begin{proof}
Consider the two summands in $\Phi_p(\ucblp_{p})$:
\begin{align*}
S_1(\ucblp_{p}) &= O(T)\, \rad\left( \ucblp_p/T,\; \tfrac{p}{d} \right), \\
S_2(\ucblp_{p}) &= O(\ucblp_p\, \tfrac{T}{B})\,\rad\left(\tfbt,\tfrac{p}{d}\right).
\end{align*}

We consider the following three cases. The first case is that
    $S_1(\ucblp_{p}) \geq \ucblp_p/12$.
Solving for $\ucblp_p$, we obtain $\ucblp_p\leq O(\frac{Td\chernoffC}{p})$, which implies that
$$ \Phi_p(\LPOPT)\geq \Omega(\ucblp_p)\geq \Omega(\LPOPT).
$$
The second case is that
    $S_2(\ucblp_{p}) \geq \ucblp_p/12$.
Then
    $$ \Phi_p(\LPOPT) \geq S_2(\LPOPT) \geq \LPOPT/12$$
In remaining case,
    $\Phi_p(\ucblp_p)\leq \frac{\ucblp_p}{6}$.
Then from Claim~\ref{cl:LP-of-Dt}(b) we get that
    $\ucblp_p\leq\, 2\,\LPOPT$.
Noting that $\Phi_p(M)$ is a non-decreasing function of $M$, we obtain
$$\Phi_p(\ucblp_p)\leq \Phi_p(2\,\LPOPT) \leq 2\,\Phi_p(\LPOPT). \qquad \qedhere
$$
\end{proof}

Now we are ready to lower-bound the LP-value for the distributions chosen by the algorithm.

\begin{claim}\label{cl:LP-phip-substitute-b}
For each distribution $\Dpx$ chosen by the algorithm in phase $p$,
$$\LP(\Dpx,\mu) \geq \LPOPT - O(\Phi_p(\LPOPT)).$$
\end{claim}

\begin{proof}
The claim follows easily from Claim~\ref{cl:LP-phip-substitute} and Claim~\ref{cl:LP-of-Dt}, noting that $\Dpx\in \F_p$.
\end{proof}

In the remainder of the analysis, denote
    $\Phi_p\triangleq \Phi_p(\LPOPT)$.
The following corollary lower-bounds the average reward; once we have it, it essentially remains to lower-bound the stopping time of the algorithm.

\begin{corollary}\label{cor:BasicBwK-Rew}
$\empir{r}_p \geq \tfrac{1}{T}\,(\LPOPT - O(\Phi_p \log p))$.
%where $\Phi_p$ denotes the right-hand side of \eqref{eq:cl:lpconvergence-Alex}.
\end{corollary}

\begin{proof}
By Claim~\ref{cl:LP-phip-substitute-b}, for each distribution $\Dqx$ chosen by the algorithm in phase $q<p$ it holds that
$$ r(\Dqx,\mu) \geq \tfrac{1}{T}\, \LP(\Dqx,\mu)
\geq \tfrac{1}{T}\, (\LPOPT - O(\Phi_q)).$$
Averaging the above equation over all rounds in phases $q<p$, we obtain
\begin{align*}
r(\aveD_p,\mu)
    &\geq \tfrac{1}{T}\, \left(
\LPOPT - \textstyle \tfrac{1}{p} \sum_{q<p} O(\Phi_q)
    \right) \\
    &\geq \tfrac{1}{T}\, \left(
        \LPOPT - O(\Phi_p \log p)
    \right).
\end{align*}
For the last inequality, we used Claim~\ref{cl:conf-rad-props}(fg) to average the confidence radii in $\Phi_q$.

Using the high-probability event in Claim~\ref{lm:high-prob-events}(c):
$$ \empir{r}_p
    \geq r(\aveD_p,\mu) - \rad( r(\aveD_p,\mu), p|X| ).
$$
Now using the monotonicity of $\nu - \rad(\nu,N)$ (Claim~\ref{cl:conf-rad-props}(c)) we obtain
\begin{align*}
\empir{r}_p
    &\geq \tfrac{1}{T}\,(\LPOPT - O(\Phi_p))
    - \rad\left(\;  \tfrac{1}{T}\,(\LPOPT - O(\Phi_p)),\; p|X| \;\right)\\
    &\geq \tfrac{1}{T}\,(\LPOPT - O(\Phi_p))
    - \rad\left(\;  \LPOPT/T,\; p|X| \;\right)\\
    &\geq \tfrac{1}{T}\,(\LPOPT - O(\Phi_p)).
\end{align*}
For the last equation, we use the fact that
$\Phi_p/T
    \geq \Omega(\rad(\LPOPT/T, \tfrac{p}{d} ))
    \geq \Omega(\rad(\;  \LPOPT/T,\; p|X| \;)).$
\end{proof}

The following two claims help us to lower-bound the stopping time of the algorithm.

\begin{claim}
\label{cl:BasicBwK-supply}
$ c_i(\Dpx,\mu) \leq \tfbt + O(1)\,\rad\left(\tfbt,\; \tfrac{p}{d} \right)$
for each resource $i$.
\end{claim}

\begin{proof}
By the algorithm's specification, $\Dpx\in \F_p$, and moreover there exists a latent structure $\mu'\in I_p$ such that $\Dpx$ is LP-perfect for $\mu'$. Apply Claim~\ref{claim:bounderror-Alex}, noting that $c_i(\Dpx,\mu') \leq \fbt$ by LP-perfectness.
\end{proof}

\begin{corollary} \label{cor:BasicBwK-supply}
    $\empir{c}_{p,i} \leq \tfbt + O(\log p)\; \rad(\tfbt, \tfrac{p}{d}) $
for each resource $i$.
\end{corollary}
\begin{proof}
Using a property of the clean execution, namely the event in Claim~\ref{lm:high-prob-events}(c), we have
\begin{align}\label{eq:cor:BasicBwK-supply-empir}
\empir{c}_{p,i}
    \leq c_i(\aveD, \mu) + \rad\left( c_i(\aveD, \mu),\; p\right).
\end{align}

Consider all rounds preceding phase $p$.
\begin{align}
 c_i(\aveD_p, \mu)
    &=  \frac{1}{p|X|}  \sum_{q<p,\, x\in X} c_i(\Dqx,\mu) & \nonumber\\
    &\leq \fbt + \frac{O(1)}{p|X|} \sum_{q<p,\, x\in X} \rad\left(\fbt, \frac{p}{d}\right)
        &\text{(by Claim~\ref{cl:BasicBwK-supply})} \nonumber\\
    &\leq \tfbt+O(\log p)\, \rad\left(\tfbt, \tfrac{p}{d}\right)
        &\text{(by Claim~\ref{cl:conf-rad-props}(fg))}.
        \label{eq:cor:BasicBwK-supply-ave}
\end{align}
For the last inequality, we used Claim~\ref{cl:conf-rad-props}(fg) to average the confidence radii.

Using the upper bound on $c_i(\aveD, \mu)$ that we derived above,
\begin{align*}
\rad\left( c_i(\aveD, \mu),\; \tfrac{p}{d}\right)
    \leq O(\log p)\; \rad\left( \tfbt+ \rad\left(\tfbt, \tfrac{p}{d}\right),\; \tfrac{p}{d} \right).
\end{align*}
Using a general property of the confidence radius that
$$ \rad(\nu+\rad(\nu,N),\,N) \leq O(\rad(\nu,N)),
$$
we conclude that
\begin{align}\label{eq:cor:BasicBwK-supply-rad}
 \rad\left( c_i(\aveD, \mu),\; \tfrac{p}{d}\right)
    \leq O(\log p)\; \rad(\tfbt, \tfrac{p}{d}).
\end{align}
We obtain the claim by plugging the upper bounds \refeq{eq:cor:BasicBwK-supply-ave} and \refeq{eq:cor:BasicBwK-supply-rad} into \refeq{eq:cor:BasicBwK-supply-empir}.
\end{proof}

We are ready to put the pieces together and derive the performance guarantee for a clean execution of \kMAB.

\begin{lemma}\label{lm:pf-Balance:almost-done}
Consider a clean execution of \kMAB. Letting $\Phi_p$ denote the right-hand side of \eqref{eq:cl:lpconvergence-Alex}, the total reward of the algorithm is
$ \Rew \geq \LPOPT - O\left( \Phi_{T/|X|}\;\log (T/|X|)\right).$
\end{lemma}
\begin{proof}
Let $p$ be the last phase in the execution of the algorithm, and let $T_0$ be the stopping time. Letting $m=|X|$, note that
    $pm <T_0 \leq (p+1)m$.

We can use Corollary \ref{cor:BasicBwK-Rew} to bound $\Rew$ from below:
\begin{align}\label{eq:pf-Balance-Rew}
\Rew
= T_0\,\empir{r}_{p+1}  > p\,m \,\empir{r}_{p+1} \geq
    \tfrac{p\,m}{T}\,(\LPOPT - O(\Phi_p \log p)).
\end{align}

Let us bound $\frac{p\,m}{T}$ from below.  The algorithm stops either when it runs out of time or if it runs out of resources during phase $p$. In the former case, $p=\flr{T/m}$. In the latter case,
    $B= T_0\,\empir{c}_{p+1,\,i} $
for some resource $i$, so
    $B\leq m(p+1)\;\empir{c}_{p+1,\,i}$.
Using Corollary \ref{cor:BasicBwK-supply}, we obtain the following lower bound on $p$:
$$ \frac{p\, m}{T}
    \geq 1 - O\left( \frac{p\, m\log p}{B} \right)\;
        \rad\left( \fbt,\, \frac{p}{d} \right).
$$
Plugging this into \eqref{eq:pf-Balance-Rew}, we conclude:
\begin{align*}
\Rew &\geq \LPOPT
    - O\left( \frac{p\, m\log p}{B} \right)\;
            \rad\left( \fbt,\, \frac{p}{d} \right) \LPOPT
    - O\left( \frac{p\,m\log p}{T} \right) \Phi_p \\
    &\geq \LPOPT - O\left( \frac{p\,m\log p}{T} \right)
        \left( \Phi_p+ \frac{T}{B}\, \rad\left( \fbt,\, \frac{p}{d} \right) \LPOPT\right)\\
  &\geq \LPOPT -\frac{p\,m\log p}{T}\; O(\Phi_p).
\end{align*}
To complete the proof, we observe that $(p\,\Phi_p \log p)$ is increasing in $p$ (by definition of $\Phi_p$), and plug in a trivial upper bound $p\leq T/m$.
\end{proof}

Using Claim~\ref{cl:conf-rad-props}(c), we can write
$$\Phi_{T/|X|}
    = O(1)\,\left(  \rad\left(\LPOPT, \tfrac{1}{d\,|X|}\right)
        + \frac{\LPOPT}{B}\; \rad\left( B, \tfrac{1}{d\,|X|}\right) \right).
$$
Rearranging the term, we obtain the bound claimed in Theorem~\ref{thm:Balance}.

\OMIT{ %%%%%%%
\ascomment{I left some Ashwin's stuff below just in case}

\ascomment{Ashwin's theorem statement}

\begin{theorem}\label{lm:basicBwK-totalrevenue}
The algorithm has total revenue
\begin{align}\label{eq-lm:basicBwK-totalrevenue}
\Rew \geq \LPOPT - O(d\, \chernoffC) \left(\frac{\maxLP}{B}\,\left(\sqrt{B |X|}+|X|\right)+\sqrt{\maxLP |X|}+|X|\right)
\end{align}
\end{theorem}

\ascomment{the last computation in Ashwin's proof}

\begin{align}\label{eq-lm:basicBwK-interface-1}
\Rew
&\geq \frac{p\, n}{T}\; \LPOPT - O(d\, \chernoffC\, n) \left(\frac{\maxLP}{B}\,\left(\sqrt{\frac{B\,p}{T}}+1\right)+\sqrt{\frac{\maxLP\,p}{T}}+1\right) \\
    &\geq \LPOPT - O(d\, \chernoffC\, n) \left(\frac{\maxLP}{B}\,\left(\sqrt{\frac{B\,p}{T}}+1\right)+\sqrt{\frac{\maxLP\,p}{T}}+1\right) \\
 &\geq \LPOPT - O(d\, \chernoffC) \left(\frac{\maxLP}{B}\,\left(\sqrt{B n}+n\right)+\sqrt{\maxLP n}+n\right)
\end{align}
} %%%%%%%%%


==> BwK-primaldualAlgorithm.tex <==
\subsection{[Deprecated!] The primal-dual algorithm (\pdbwk)}
\label{sec:pd-bwk-alg}

%
% this paragraph is pretty good.
% but reword it to emphasize the ``bang-per-buck'' interpretation
% in connection with this, remind the reader of the proof that
%   the opt dynamic policy can't do better than the lp-opt.

This section develops an algorithm, called \pdbwk, that solves the \BwK problem
using a very natural and intuitive idea: greedily select arms
with the greatest estimated ``bang per buck,'' i.e.\ reward per unit
of resource consumption. One of the main difficulties with this
idea is that there is no such thing as a ``unit of resource consumption'':
there are $\nrsc$ different resources, and it is
unclear how to trade off consumption of one resource
versus another. The proof of Lemma~\ref{lem:lp-relax}
gives some insight into how to quantify this trade-off:
an optimal dual solution $\eta^*$ can be interpreted
as a vector of unit costs for resources, such that for every
arm the expected reward is less than or equal to the expected
cost of resources consumed. Since our goal is to match the
optimum value of the LP as closely as possible, we must minimize
the shortfall between the expected reward of the arms we pull
and their expected resource cost as measured by $\eta^*$.
Thus, our algorithm will try to learn an optimal dual
vector $\eta^*$ in tandem with learning
the latent structure $\mu$.

Borrowing an idea from \citep{AroraHK,GargK,PlotkinST}, we will
use the multiplicative weights update method to learn the
optimal dual vector. This method raises the cost of a resource
exponentially as it is consumed, which ensures that heavily demanded
resources become costly, and thereby promotes balanced
resource consumption. Meanwhile, we still have to ensure
(as with any multi-armed bandit problem) that our algorithm
explores the different arms frequently enough to gain adequately accurate
estimates of the latent structure. We do this by estimating
rewards and resource consumption as optimistically as possible,
i.e.\ using upper confidence bound (UCB) estimates for rewards and
lower confidence bound (LCB) estimates for resource consumption.
Although both of these techniques --- multiplicative weights and
confidence bounds --- have both successfully applied in previous
online learning algorithms, it is far from obvious that this
particular hybrid of the two methods should be effective. In
particular, the use of multiplicative updates on dual
variables, rather than primal ones, distinguishes our algorithm
from other bandit algorithms that use multiplicative weights
(e.g. the $\expthree$ algorithm \citep{bandits-exp3}) and brings
it closer in spirit to the literature on stochastic packing
algorithms (especially \citep{DevanurJSW-ec11}).

The pseudocode for the algorithm is presented below. When we refer to the UCB or LCB for a latent parameter
(the reward of an arm, or the amount of some resource that it utilizes),
these are computed as follows. Letting $\hat{\nu}$ denote the empirical
average of the observations of that random variable\footnote{Note
that we initialize the
algorithm by pulling each arm once, so empirical averages
are always well-defined.} and letting $N$ denote the number of times
the random variable has been observed, the lower confidence bound
(LCB) and upper confidence bound (UCB) are the left and right endpoints,
respectively, of the \emph{confidence interval} $[0,1] \cap
[\hat{\nu} - \rad(\hat{\nu},N), \; \hat{\nu} + \rad(\hat{\nu},N)]$.
The UCB or LCB for a vector or matrix are defined componentwise.

\begin{comment} % AS(2014-11-24) no need for this explanation with the new pseudocode
In step~\ref{algstep:argmin}, the pseudocode asserts that the
set $\argmin_{\x \in \splx{\armset}}
\{ \frac{y_t^\trans \clcb{t} \x}{\rucb{t}^\trans \x} \}$
contains at least one of the point-mass distributions
$\{ \sbv_1,\ldots,\sbv_{\narms} \}$. This is true, because
if $\rho = \min_{\x \in \splx{\armset}}
\{ (y_t^\trans \clcb{t} \x)/(\rucb{t}^\trans \x) \}$
then the linear inequality $y_t^\trans \clcb{t} \x \leq \rho \rucb{t}^\trans \D$
holds at some point $\x \in \splx{\arms}$, and
hence it holds at some extreme point, i.e.\ one of the
point-mass distributions.
\end{comment}

\newcommand{\EstCost}{\mathtt{EstCost}}

\begin{algorithm}[H]
\myCaption{\pdbwk}
%\label{alg:pdbwk}
\begin{algorithmic}[1]
\STATE {\bf Initialization}
\STATE \TAB In the first $\narms$ rounds, pull each arm once.
\STATE \TAB $v_1 = \ones \in [0,1]^\nrsc$.
\STATE \TAB\TAB
    \COMMENT{$v_t\in [0,1]^\nrsc$ is the round-$t$ estimate of the optimal solution $\eta^*$ to \refeq{lp:dual} in Section~\ref{sec:lp}.}
\STATE \TAB\TAB
    \COMMENT{We interpret $v_t(i)$ as an estimate of the (fictional) unit cost of  resource $i$, for each $i$.}
\STATE \TAB Set $\eps = \sqrt{\ln(\nrsc)/\budg}$.
\FOR{rounds $t = \narms+1,\ldots,\stime \;\; \mbox{\it (i.e., until
resource budget exhausted)}$}
\STATE For each arm $x\in X$,
\STATE \TAB Compute UCB estimate for the expected reward, $\rucb{t,x} \in [0,1]$.
\STATE \TAB Compute LCB estimate for the resource consumption vector,
                $\clcb{t,x} \in [0,1]^{\nrsc}$.
\STATE \TAB \emph{Expected cost} for one pull of arm $x$ is estimated by $\EstCost_x = \clcb{t,x}\cdot v_t$.
\STATE Pull arm $x=x_t\in X$ that maximizes  $\rucb{t,x}/\EstCost_x$,
            the optimistic \emph{bang-per-buck} ratio.
\label{algstep:argmin}
\STATE Update estimated unit cost for each resource $i$:
\begin{align*}
                v_{t+1}(i) = v_t(i)\, (1+\eps)^{\ell},\;  \ell = \clcb{t,x}(i).
\end{align*}
\label{algstep:mwu}
\ENDFOR
\end{algorithmic}
\end{algorithm}

%\ascomment{Bobby's original pseudocode -- will remove.}
%\begin{algorithm}[H]
%\myCaption{\pdbwk}
%%\label{alg:pdbwk}
%\begin{algorithmic}[1]
%\STATE Set $\eps = \sqrt{\ln(\nrsc)/\budg}$.
%\STATE In the first $\narms$ rounds, pull each arm once.
%\STATE $v_1 = \ones$
%% \STATE $t=\narms+1$
%\FOR{$t = \narms+1,\ldots,\stime \;\; \mbox{\it (i.e., until
%resource budget exhausted)}$}
%\STATE Compute UCB estimate for reward vector, $\rucb{t}$.
%\STATE Compute LCB estimate for resource consumption matrix, $\clcb{t}$.
%\STATE $y_t = v_t / (\ones^\trans v_t)$.
%\STATE Pull arm $x_j$ such that point-mass distribution
%$\x_t = \sbv_j$ belongs to $\argmin_{\x \in \splx{\armset}}
%\{ \frac{y_t^\trans \clcb{t} \x}{\rucb{t}^\trans \x} \}$.
%%\label{algstep:argmin}
%% \STATE Pull an arm from point distribution $\x_t$
%\STATE $v_{t+1} = \diag{(1+\eps)^{\sbv_j^\trans L_t \x_t}} v_t$.
%\label{algstep:mwu}
%% \STATE $t = t+1$.
%\ENDFOR
%\end{algorithmic}
%\end{algorithm}

%Another feature of our algorithm that deserves mention
We use a variant of the Garg-K\"onemann width
reduction technique \citep{GargK}. The ratio
%$(y_t^\trans \clcb{t} \x_t)/(\rucb{t}^\trans \x_t)$
$\rucb{t,x}/\EstCost_x$
that we optimize in step~\ref{algstep:argmin} may
be unboundedly large, so in the multiplicative update
in step~\ref{algstep:mwu} we rescale this value to
%$y_t^\trans \clcb{t} \x_t$,
$\clcb{t,x}(i)$,
which is guaranteed
to be at most 1;
this rescaling is mirrored in the
analysis of the algorithm.
% (when we define the dual vector $\bar{y}$).
% by averaging the vectors $y_t$
%using the aforementioned scale factors.
Interestingly, unlike the Garg-K\"onemann algorithm which
applies multiplicative updates to the dual
vectors and weighted averaging to the primal ones,
in our algorithm the multiplicative updates
and weighted averaging are \emph{both} applied to
the dual vectors.

%% In this section we present an algorithm for \BwK based on Multiplicative weight updates(MWU) method. There are two interesting ideas in our application of MWU. One of them is that we maintain a dual vector and update it using MWU. The intuitive reasoning as to why this should help is that this helps prioritize which resource is getting consumed at a faster rate. If one of the resources is consumed more then the dual variable corresponding to that particular constraint is larger which results in the algorithm choosing an arm which uses less of that particular resource. This argument is only at an intuitive level since each arm could potentially consume more than one resource. The other interesting idea is the combination of UCB type of analysis with primal-dual type of analysis. Towards this end we use most optimistic estimates for different parameters (UCB for revenue and LCB for resource).

%
% in this paragraph it's important to explain how we're doing
%   something similar to Garg-Konemann, but not quite the same.
%   (G-K applies MW to dual and weighted averaging to primal.)
%   (We apply MW and weighted averaging both to dual.)

%% The algorithm maintains a dual (possibly infeasible) solution $y_t$ and does MWU on it. In each round it computes ``optimistic" estimate for parameters related to each arm. This is UCB estimates for vector of rewards $\rucb{t}$ and LCB estimates for the resource consumption matrix $\clcb{t}$. Then it chooses to ``pull" an arm based on maximizing a function based on the estimates and the current dual solution and finally updates the dual solution using multiplicative weight update.

%
% also need to say somewhere how confidence intervals are computed
% in this algorithm!

The algorithm is fast: with machine word size of $\log T$ bits or more, the per-round running time is $O(\narms \nrsc)$. Moreover, if each arm $x$ consumes only $\nrsc_x$ resources that are known in advance, then $\clcb{t,x}$ can be implemented as a $\nrsc_x$-dimensional vector, and $\EstCost_x$ can be computed in $O(\nrsc_x)$ time. Then the per-round running time is
    $O(\narms + \nrsc+\sum_x \nrsc_x)$.


The following theorem expresses the regret guarantee
for \pdbwk. The proof is in Section~\ref{sec:pdbwk-analysis}.
\begin{theorem} \label{thm:pdbwk}
Consider an instance of \BwK with $d$ resources, $m=|X|$ arms, and the smallest budget $B = \min_i B_i$.
%For any instance of the \BwK problem,
The regret of algorithm \pdbwk satisfies
\begin{equation} \label{eq:pdbwk-regret}
\LPOPT -\algrwd
\leq
O \left( \sqrt{\log(\nrsc \horizon)}\right)
\left( \sqrt{\narms \, \LPOPT} + \LPOPT \, \sqrt{\frac{\narms}{\budg}} \right)\;
+ O(\narms)\, \log(\nrsc \horizon)\log(\horizon).
\end{equation}
Moreover, \eqref{eq:regret-LPOPT-OPT} holds with $f(\LPOPT)$ equal to the right-hand side of \eqref{eq:pdbwk-regret}.
\end{theorem}

\OMIT{ %%%%%%%%
\noindent Comparing this bound to Theorem~\ref{thm:Balance},
when $\nrsc = O(1)$ and $\maxLP = O(\optrwd)$ the two
guarantees are the same up to logarithmic factors.
The regret guarantee for the primal-dual algorithm
scales better with the number of resources, $\nrsc$,
and it can be vastly superior in cases where
$\optrwd \ll \maxLP$.

In fact, we prove a slightly stronger regret bound:

\begin{theorem} \label{thm:pdbwk-LP}
For any instance of the \BwK problem,
the reward of Algorithm \pdbwk satisfies
\begin{equation} \label{eq:pdbwk-regret-LP}
\algrwd \geq \LPOPT-f(\LPOPT) \geq \OPT-f(\OPT),
\end{equation}
where $f(\OPT)$ denotes the right-hand side of \eqref{eq:pdbwk-regret}.
\end{theorem}

Note that the regret bound relative to $\LPOPT$ has the square-root scaling property:  if all budget constraints, including the time horizon, are increased by the factor of $\alpha$, then the regret bound $f(\LPOPT)$ scales as $\sqrt{\alpha}$. (According to the lower bound proved in \citet{bandits-exp3}, this scaling is optimal even for the basic MAB problem.)
} %%%%%%%


==> BwK-primaldualAnalysis.tex <==
\section{[Deprecated!] Analysis of \pdbwk (Proof of Theorem~\ref{thm:pdbwk})}
%\label{sec:det-rewd}
\label{sec:pdbwk-analysis}

In this section we present the analysis of the
$\pdbwk$ algorithm. We begin by recalling
the $\hdg$ algorithm~\cite{FS97} from online learning theory,
and its performance guarantee. Next, we present
a simplified analysis of $\pdbwk$ in a toy model
in which the outcome vectors are deterministic.
(This toy model of the \BwK problem is uninteresting
as a learning problem since the latent structure
does not need to be learned, and the problem reduces
to solving a linear program. We analyze $\pdbwk$ first
in this context because the analysis is simple, yet
its main ideas carry over to the general case which
is more complicated.)

Throughout this section, it will be useful
to represent the latent values as matrices and vectors. For this purpose, we will number the arms as $\arms = \{ 1 \LDOTS \narms \}$ and let $r \in \R^{\narms}$
denote the vector whose $x$-th component is $r(x,\mu)$, the expected reward, for each arm $x\in X$. Similarly we will let $C \in \R^{\nrsc \times \narms}$ denote the matrix whose
$(i,x)$ entry is $c_i(j,\mu)$, the expected resource consumption, for each resource $i$ and each arm $x$. Let $\sbv_j^d\in \{0,1\}^d$ denote the $d$-dimensional $j$-th coordinate vector.


\subsection{The $\hdg$ algorithm}
\label{sec:hedge}

In this section we present the $\mathsf{Hedge}$
algorithm from \citet{FS97}, also known as the multiplicative weights
algorithm. It is an online algorithm for maintaining
a $d$-dimensional probability vector $y$ while
observing a sequence of
$d$-dimensional payoff vectors $\pi_1,\ldots,\pi_\stime$.
The algorithm is initialized with a parameter
$\eps \in (0,1)$.
The version presented below, along with the
following performance guarantee, is adapted from \citet{cs683week2}.

\begin{algorithm}[H]
\myCaption{$\mathsf{Hedge}(\eps)$}
%\label{alg:hdg}
\begin{algorithmic}[1]
\STATE $v_1 = \ones$
    \TAB\COMMENT{$v_t \in \R^d_+$ for each round $t$.}
\FOR{$t=1,2,\ldots,\stime$}
\STATE $y_t = v_t / \| v_t \|_1$.
\FOR{each resource $i$}
\STATE $v_{t+1}(i) = v_t(i)\, (1+\eps)^\ell$, $\ell = \pi_{t}(i)$.
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

%\ascomment{Bobby's orignal pseudocode. Will remove.}
%\begin{algorithm}[H]
%\myCaption{$\mathsf{Hedge}(\eps)$}
%%\label{alg:hdg}
%\begin{algorithmic}[1]
%\STATE $v_1 = \ones$
%\FOR{$t=1,2,\ldots,\stime$}
%\STATE $y_t = v_t / (\ones^\trans v_t)$.
%\STATE $v_{t+1} = \diag{(1+\eps)^{\pi_{ti}}} v_t$.
%\ENDFOR
%\end{algorithmic}
%\end{algorithm}


\begin{proposition} \label{prop:hedge}
For any $0 < \eps < 1$ and any sequence of payoff
vectors $\pi_1,\ldots,\pi_\stime \in [0,1]^d$, we have
\[
\forall y \in \splx{d} \quad
\sum_{t=1}^\stime y_t^\trans \pi_t \geq (1-\eps) \sum_{t=1}^\stime y^\trans \pi_t
- \frac{\ln d}{\eps}.
\]
\end{proposition}
\noindent
A self-contained proof of the proposition, for the reader's convenience,
appears in Appendix~\ref{app:hedge}.

\subsection{Warm-up: The deterministic case}
\label{sec:pdbwk-determ}

To present the application of $\hdg$ to \BwK
in its purest form, we first present
an algorithm for the case in which the rewards
of the various arms are deterministically equal
to the components of a vector $r \in \R^{\narms}$,
and the resource consumption vectors are deterministically
equal to the columns of a matrix $C \in \R^{\nrsc \times \narms}$.

\begin{algorithm}[H]
\caption{Algorithm \pdbwk, adapted for deterministic outcomes}
\label{alg:determ}
\begin{algorithmic}[1]
\STATE {\bf Initialization}
\STATE \TAB In the first $\narms$ rounds, pull each arm once.
\STATE \TAB For each arm $x\in X$, let $r_x\in [0,1]$ and $C_x\in[0,1]^d$
\STATE \TAB\TAB denote the reward and the resource consumption vector revealed in Step 2.
\STATE \TAB $v_1 = \ones \in [0,1]^\nrsc$.
\STATE \TAB\TAB
    \COMMENT{$v_t\in [0,1]^\nrsc$ is the round-$t$ estimate of the optimal solution $\eta^*$ to \refeq{lp:dual} in Section~\ref{sec:lp}.}
\STATE \TAB\TAB
    \COMMENT{We interpret $v_t(i)$ as an estimate of the (fictional) unit cost of  resource $i$, for each $i$.}
\STATE \TAB Set $\eps = \sqrt{\ln(\nrsc)/\budg}$.
\FOR{rounds $t = \narms+1,\ldots,\stime \;\; \mbox{\it (i.e., until
resource budget exhausted)}$}
\STATE For each arm $x\in X$,
\STATE \TAB \emph{Expected cost} for one pull of arm $x$ is estimated by $\EstCost_x = C_x\cdot v_t$.
\STATE Pull arm $x=x_t\in X$ that maximizes  $r_x/\EstCost_x$, the \emph{bang-per-buck} ratio.
\label{algstep:argmin-det}
\STATE Update estimated unit cost for each resource $i$:
\begin{align*}
                v_{t+1}(i) = v_t(i)\, (1+\eps)^{\ell},\;  \ell = C_x(i).
\end{align*}
\ENDFOR
\end{algorithmic}
\end{algorithm}

%\ascomment{Bobby's orignal pseudocode. Will remove.}
%\begin{algorithm}[H]
%\caption{Algorithm \pdbwk, adapted for deterministic outcomes}
%%\label{alg:determ}
%\begin{algorithmic}[1]
%\STATE In the first $\narms$ rounds, pull each arm once.
%\STATE
%Let $r,\, C$ denote the reward vector and resource consumption matrix
%revealed in Step 1.
%\STATE $v_1 = \ones$
%\STATE $t=1$
%\FOR{$t = \narms+1,\ldots,\stime \;\; \mbox{\it (i.e., until
%resource budget exhausted)}$}
%\STATE $y_t = v_t / (\ones^\trans v_t)$.
%\STATE Pull arm $x_j$ such that point-mass distribution
%$\x_t = \sbv_j$ belongs to
%$\argmin_{\x \in \splx{\armset}} \{ \frac{y_t^\trans C \x}{r^\trans \x} \}$.
%\STATE $v_{t+1} = \diag{(1+\eps)^{\sbv_j^\trans C \x_t}} v_t$.
%\STATE $t = t+1$.
%\ENDFOR
%\end{algorithmic}
%\end{algorithm}

This algorithm is an instance of the multiplicative-weights
update method for solving packing linear programs. Interpreting
it through the lens of online learning, as in the survey \citet{AroraHK},
it is updating a vector $y_t = v_t / \| v_t \|_1$ using
the $\hdg$ algorithm, were the payoff vector in any round $t$ is given by $C_{x_t}$.
%Note that these payoffs belong to $[0,1]$, by our
%assumption that $C$ has $[0,1]$ entries.

Let $\xi^*$ denote an optimal solution of the primal linear
program~\refeq{lp:primal} from Section~\ref{sec:lp},
and let $\optlp = r^\trans \xi^*$ denote the optimal
value of that LP.

For each round $t$, let $\x_t = \sbv_{x_t}^\narms$ denote the $x_t$-th coordinate vector.
We claim
\begin{align}\label{eq:PDBwK-pointmass-det}
z_t \in \argmax_{\x \in \splx{\armset}} \left\{ \frac{r^\trans \x}{y_t^\trans C \x} \right\}.
\end{align}
In words: $z_t$ maximizes the ``bang-per-buck ratio" among all distributions $z$ over arms. Indeed, the  $\argmax$ in \eqref{eq:PDBwK-pointmass-det} is well-defined as that of a continuous function on a compact set. Say it is attained by some distribution $z$ over arms, and let $\rho\in\R$ be the corresponding $\max$. By maximality of $\rho$, the linear inequality
    $ \rho\, y_t^\trans C \x \geq r^\trans \x $
also holds at some extremal point of the probability simplex $\splx{\armset}$, i.e. at some point-mass distribution. For any such point-mass distribution, the corresponding arm maximizes the bang-per-buck ratio in the algorithm. Claim proved.

Let $\algrwd = \sum_{t=\narms+1}^{\stime-1} r^\trans \x_t$ denote the
total payoff obtained by the algorithm after its initialization phase
(the first $\narms$ rounds).
Let $y=\sbv_i^\nrsc$, where $i$ is a resource exhausted by the algorithm when it stops; then
    $y^\trans C \left(\sum_{t=1}^\stime \x_t \right) \geq \budg$.
Note that the algorithm's
initialization phase consumes at most $\narms$ units of any resource,
and the final round $\stime$ consumes at most one unit more, so
\begin{equation} \label{eq:determ.1}
y^\trans C \left( \sum_{\narms < t < \stime} \x_t \right) \geq \budg - \narms - 1.
\end{equation}
Finally, let
\[
\bar{y} = \frac{1}{\algrwd} \sum_{\narms<t<\stime} (r^\trans \x_t) y_t.
\]


Now we have
\begin{align*}
\budg & \geq \bar{y}^\trans C \xi^* = \frac{1}{\algrwd}
\sum_{\narms < t < \stime} (r^\trans \x_t)(y_t^\trans C \xi^*) \\
&\geq \frac{1}{\algrwd} \sum_{\narms < t < \stime} (r^\trans \xi^*) (y_t^\trans C \x_t) \\
&\geq \frac{\optlp}{\algrwd} \left[
(1-\eps) \sum_{\narms < t < \stime} y^\trans C \x_t - \frac{\ln \nrsc}{\eps} \right] \\
&\geq \frac{\optlp}{\algrwd} \left[ \budg - \eps \budg - \narms - 1 - \frac{\ln \nrsc}{\eps} \right].
\end{align*}
The first inequality is by primal feasibility of $\xi^*$,
the second is by \eqref{eq:PDBwK-pointmass-det},
% the definition of $\x_t$,
the third is the performance guarantee of Hedge, the fourth is
by~\refeq{eq:determ.1}.
Putting these inequalities together we have derived
\[
\frac{\algrwd}{\optlp} \geq 1 - \eps - \frac{\narms+1}{\budg} -
\frac{\ln \nrsc}{\eps \budg}.
\]
Setting $\eps = \sqrt{\frac{\ln \nrsc}{\budg}}$ we find
that the algorithm's regret is bounded above by
$\optlp \cdot O \left( \sqrt{\frac{\ln \nrsc}{\budg}} + \frac{\narms}{\budg}
\right).$

\subsection{Analysis modulo error terms}
\label{sec:modulo-errors}

We now commence the analysis of Algorithm \pdbwk.
In this section we show how to reduce the problem
of bounding the algorithm's regret to a problem
of estimating two error terms that reflect the
difference between the algorithm's confidence-bound estimates
of its own reward and resource consumption with the
empirical values of these random variables.
The analysis of those error terms will be the subject
of Section~\ref{sec:error-analysis}.

Recall that the algorithm computes LCBs on expected resource consumption $\clcb{t,x}\in [0,1]^\nrsc$ and UCBs on expected rewards $\rucb{t,x}\in [0,1]$, for each round $t$ and each arm $x$. We also represent the LCBs as a matrix
    $\clcb{t} \in [0,1]^{\nrsc \times \narms}$
whose $x$-th column equals $\clcb{t,x}$, for each arm $x$. We also represent the UCBs as a vector $\rucb{t}\in [0,1]^\narms$ over arms whose $x$-th component equals $\rucb{t,x}$.

As in the previous subsection, let $\x_t = \sbv_{x_t}^\narms$ denote the $x_t$-th coordinate vector, and let
    $y_t = v_t / \| v_t \|_1$.
Similar to \eqref{eq:PDBwK-pointmass-det}, $z_t$ maximizes the ``bang-per-buck ratio" among all distributions $z$ over arms:
\begin{align}\label{eq:PDBwK-pointmass}
z_t \in \argmax_{\x \in \splx{\armset}} \left\{ \frac{\rucb{t,x}^\trans \x}{y_t^\trans \clcb{t,x}\, \x} \right\}.
\end{align}

By Theorem~\ref{thm:conf-rad} and our choice of $\chernoffC$, it
holds with probability at least $1-T^{-1}$ that the confidence interval
for every latent parameter, in every round of execution, contains
the true value of that latent parameter. We call this high-probability
event a \emph{clean execution} of \pdbwk. Our regret guarantee will
hold deterministically assuming that a clean execution takes place.
The regret can be at most $T$ when a clean execution does not take
place, and since this event has probability at most $T^{-1}$ it
contributes only $O(1)$ to the regret. We will henceforth assume
a clean execution of \pdbwk.

Let $C_t$ be the resource-consumption matrix for round $t$. That is,
    $C_t \in [0,1]^{\nrsc \times \narms}$
denotes the matrix whose $(i,x)$ entry is the actual consumption of resource $i$ in round $t$ if arm $x$ were chosen in this round.

\begin{claim}\label{cl:modulo-errors}
% When Algorithm \pdbwk is run with parameter
%         $\eps = \sqrt{\frac{\ln \nrsc}{B}}$
% its expected total reward satisfies the bound:
In a clean execution of Algorithm \pdbwk, the algorithm's
total reward satisfies the bound
\begin{equation} \label{eq:modulo-errors}
\algrwd \geq \optlp - \left[
  2 \optlp \left( \sqrt{\frac{\ln \nrsc}{\budg}} +
                \frac{\narms + 1}{\budg} \right) +
  \narms + 1 \right] -
  \frac{\optlp}{\budg} \left\| \sum_{\narms<t<\stime} \cdif{t} \x_t \right\|_\infty -
  \left| \sum_{\narms<t<\stime} \rdif{t}^\trans \x_t \right|,
\end{equation}
where $\cdif{t}$ and $\rdif{t}$ are defined by
\begin{equation} \label{eq:etrt}
\cdif{t} = \crlz{t} - \clcb{t}, \qquad
\rdif{t} = \rucb{t} - \rrlz{t}.
\end{equation}
\end{claim}

\begin{proof}
The claim is proven by mimicking the analysis of
Algorithm~\ref{alg:determ} in the preceding section,
incorporating error terms that reflect the differences
between observable values and latent ones.
%% The analysis of the algorithm parallels the analysis in the fully
%% deterministic case, while incorporating error terms that
%% reflect the differences between the matrices $\clcb{t}, \crlz{t}$, and $C$,
%% and similarly for the vectors $\rucb{t}, \rrlz{t}, r$.
%% For example, the stopping condition for the algorithm is now expressed
%% by the fact that $y^\trans \sum_{t=1}^\stime \crlz{t} \x_t \geq \budg$,
%% rather than $y^\trans C \sum_{t=1}^\stime \x_t \geq \budg$.
As before, let $\xi^*$ denote an optimal solution of the primal linear
program~\refeq{lp:primal},
and let $\optlp = r^\trans \xi^*$ denote the optimal value of that LP.
Let $\optucb = \sum_{\narms < t < \stime} \rucb{t}^\trans \x_t$ denote the
total payoff the algorithm would have obtained, after its initialization
phase, if the actual
payoff at time $t$ were replaced with the upper confidence bound.
Let $y=\sbv_i^\nrsc$, where $i$ is a resource exhausted by the algorithm when it stops; then
    $y^\trans \left(\sum_{t=1}^\stime \crlz{t} \x_t \right) \geq \budg$.
As before,
\begin{equation} \label{eq:pdbwk.1}
y^\trans \left( \sum_{\narms < t < \stime} \crlz{t} \x_t \right) \geq \budg - \narms - 1.
\end{equation}
Finally let
\[
\bar{y} = \frac{1}{\optucb} \sum_{\narms < t < \stime} (\rucb{t}^\trans \x_t) y_t.
\]
Assuming a clean execution, we have
{\allowdisplaybreaks
\begin{align}
\budg & \geq \bar{y}^\trans C \xi^*
  && \mbox{\it ($\xi^*$ is primal feasible)}
\nonumber \\
  &= \frac1{\optucb} \sum_{\narms < t < \stime}
     (\rucb{t}^\trans \x_t)(y_t^\trans C \xi^*)
 &&
\nonumber \\
  & \geq \frac{1}{\optucb} \sum_{\narms<t<\stime} (\rucb{t}^\trans \x_t) (y_t^\trans \clcb{t} \xi^*)
 && \mbox{\it (clean execution)}
\nonumber \\
  & \geq \frac{1}{\optucb} \sum_{\narms<t<\stime} (\rucb{t}^\trans \xi^*) (y_t^\trans \clcb{t} \x_t)
 && \mbox{\it (by \eqref{eq:PDBwK-pointmass})}
\nonumber \\
  & \geq \frac{1}{\optucb} \sum_{\narms<t<\stime} (r^\trans \xi^*) (y_t^\trans \clcb{t} \x_t)
 && \mbox{\it (clean execution)}
\nonumber \\
  & \geq \frac{\optlp}{\optucb} \left[
         (1 - \eps) y^\trans \left( \sum_{\narms<t<\stime} \clcb{t} \x_t \right)
         - \frac{\ln \nrsc}{\eps} \right]
 && \mbox{\it (Hedge guarantee)}
\nonumber \\
  & = \frac{\optlp}{\optucb} \left[
           (1-\eps) y^\trans \left( \sum_{\narms<t<\stime} \crlz{t} \x_t \right)
         - (1-\eps) y^\trans \left( \sum_{\narms<t<\stime} \cdif{t} \x_t \right)
         - \frac{\ln \nrsc}{\eps} \right]
 &&
\nonumber \\
  & \geq \frac{\optlp}{\optucb} \left[
           (1-\eps) \budg - \narms - 1
         - (1-\eps) y^\trans \left( \sum_{\narms<t<\stime} \cdif{t} \x_t \right)
         - \frac{\ln \nrsc}{\eps} \right]
 && \mbox{\it (definition of $y$; see eq.~\refeq{eq:pdbwk.1})}
\nonumber \\
\optucb
  & \geq \optlp \left[ 1 - \eps - \frac{\narms+1}{\budg} -
         \frac{1}{\budg} \left\| \sum_{\narms<t<\stime} \cdif{t} \x_t \right\|_{\infty}
         - \frac{\ln \nrsc}{\eps \budg} \right] .
  &&
\label{eq:optucb}
%% \nonumber \\
%%   & \geq \optlp \left[ 1 - \eps - \frac{2(\narms+1)}{\budg} -
%%          \frac{1}{\budg} \left\| \sum_{t=1}^{\stime} \cdif{t} \x_t \right\|_{\infty}
%%          - \frac{\ln \nrsc}{\eps \budg} \right] .
%%   && \mbox{\it (since $\|E_t \x_t\|_\infty \leq 1$ for all $t$)}
\end{align}
} % END \allowdisplaybreaks
The algorithm's actual payoff,
    $\algrwd = \sum_{t=1}^\stime \rrlz{t}^\trans \x_t$,
satisfies the inequality
    $$\algrwd \geq
            \optucb - \sum_{\narms<t<\stime} (\rucb{t} - \rrlz{t})^\trans \x_t
          = \optucb - \sum_{\narms<t<\stime} \rdif{\stime}^\trans \x_t.
    $$
Combining this inequality with~\refeq{eq:optucb},
%% Finally, comparing the definition of $\optucb$ to the algorithm's
%% actual payoff, $\algrwd = \sum_{t=1}^\stime \rrlz{t}^\trans \x_t$,
%% we have
%% \begin{align}
%% \algrwd
%%    & \geq \optucb - \sum_{\narms<t<\stime} (\rucb{t} - \rrlz{t})^\trans \x_t
%% \nonumber \\
%%    & = \optucb - \sum_{t=1}^\stime \rdif{t}^\trans \x_t +
%%        \left( \sum_{t=1}^\narms \rdif{t}^\trans \x_t
%%               + \rdif{\stime}^\trans \x_\stime \right)
%% \nonumber \\
%%    & \geq \optucb - \narms - 1 -
%%      \left| \sum_{t=1}^\stime \rdif{t}^\trans x_t \right|
%% \label{eq:algrwd}
%% \end{align}
%% Combining~\refeq{eq:optucb} and~\refeq{eq:algrwd} we obtain
we obtain the bound~\refeq{eq:modulo-errors}, as claimed.
\end{proof}

\subsection{Error analysis}
\label{sec:error-analysis}

In this section we complete the proof of Theorem~\ref{thm:pdbwk}
by deriving upper bounds on the terms
$\left\| \sum_{\narms<t<\stime} \cdif{t} \x_t \right\|_\infty$
and $\left| \sum_{\narms<t<\stime} \rdif{t} \x_t \right|$
appearing on the right side of~\refeq{eq:modulo-errors}.
Both bounds are special cases of a more
general statement, presented as Lemma~\ref{lem:vector-conf} below.
Before stating the lemma, we need to establish
a simple fact about confidence radii.

\begin{lemma} \label{lem:confrad-sum}
For any two vectors $a,N \in \R_+^\narms$, we have
\begin{equation} \label{eq:confrad-sum}
\sum_{j=1}^{\narms} \rad(a_j,N_j) \, N_j \leq
\sqrt{\chernoffC \, m (a^\trans N)} + \chernoffC \, m.
\end{equation}
\end{lemma}
\begin{proof}
The definition of $\rad(\cdot,\cdot)$ implies that
$\rad(a_j,N_j) \, N_j \leq \sqrt{\chernoffC \, a_j N_j} + \chernoffC$.
Summing these inequalities and applying Cauchy-Schwarz,
\[
\sum_{j=1}^{\narms} \rad(a_j,N_j) \, N_j \leq
\sum_{j=1}^{\narms} \sqrt{\chernoffC \, a_j N_j} + \chernoffC\, m \leq
\sqrt{m} \cdot \sqrt{\sum_{j \in \arms} \chernoffC \,  a_j N_j} + \chernoffC\, m,
\]
and the lemma follows by rewriting the expression on the right side.
\end{proof}

The next lemma requires some notation and definitions.
Suppose that $a_1,\ldots,a_\stime$ is a sequence of vectors
in $[0,1]^\narms$ and that $\x_1,\ldots,\x_\stime$ is a sequence
of vectors in
    $\{\sbv^\narms_1 \LDOTS \sbv^\narms_\narms\}$.
Assume that the
latter sequence begins with a permutation of the elements of
    $\{\sbv^\narms_1 \LDOTS \sbv^\narms_\narms\}$
so that, for every round $s \geq \narms$,
the diagonal matrix $\sum_{t=1}^s \x_t \x_t^\trans$ is invertible.
The vector
\[
\aemp{s} = \left( \sum_{t=1}^s \x_t \x_t^\trans \right)^{-1}
\left( \sum_{t=1}^s \x_t \x_t^\trans a_t \right) \in [0,1]^\narms
\]
can be interpreted as the vector of empirical averages over arms: for each arm $j$,
the entry $\aemp{s,j}$ is equal to the average of
$a_{t,j}$ over all times $t \leq s$ such that $\x_t=\sbv_j^\narms$
(intuitively: over the times $t \leq s$ when arm $j$ has been played).
Let $\vnpul_s = \sum_{t=1}^s \x_t \in \N^\narms$ denote the vector over arms
whose $j$-th entry equals
%entry $\vnpul_{s,j}$ indicates
the number of times $\sbv_j$ occurs in the sequence $\x_1,\ldots,\x_s$
(intuitively: the number of times arm $j$ was played up to and including round $s$).
A useful identity is
\[
\aemp{t}^\trans \vnpul_t = \sum_{s=1}^t a_s^\trans \x_s.
\]
%% Define
%% the vector of confidence radii $\arad{t}$ by specifying that
%% $\arad{t,j} = \rad(\aemp{t,j},\npul_{t,j})$.
\begin{lemma} \label{lem:vector-conf}
Suppose we are given sequences of vectors $a_1,\ldots,a_\stime$
and $\x_1,\ldots,\x_\stime$ as above. Suppose we are additionally given
a sequence of vectors $b_1,\ldots,b_\stime$ in $[0,1]^\narms$
and another vector $a_0$
such that for $\narms < t < \stime$ and $j \in \arms$,
$$|b_{t,j} - a_{0,j}| \leq 2 \, \rad(\aemp{t,j},\npul_{t,j}) \leq
6 \, \rad(a_{0,j}, \npul_{t,j}).$$
Let $s=\stime-1$ and suppose that for all $j \in \arms$,
$|\aemp{s,j} - a_{0,j}| \leq \rad(\aemp{s,j},\npul_{s,j})$.
Then
\begin{equation} \label{eq:vector-conf}
\left| \sum_{\narms < t < \stime} (b_t - a_t)^\trans \x_t \right| \leq
O \left( \sqrt{\chernoffC \, \narms \asum} + \chernoffC \, \narms\, \log\horizon \right),
\end{equation}
where $\asum = (\aemp{\stime-1})^{\trans} \vnpul_{\stime-1}
= \sum_{t=1}^{\stime-1} a_t^\trans \x_t$.
\end{lemma}
\begin{proof}
Decompose the left side of~\refeq{eq:vector-conf}
as a sum of three terms,
\begin{equation} \label{eq:vc.1}
\sum_{\narms < t < \stime} (b_t - a_t)^\trans \x_t =
\sum_{t=1}^{\narms} (a_t - b_t)^\trans \x_t +
\sum_{t=1}^{\stime-1} (b_t - a_0)^\trans \x_t +
\sum_{t=1}^{\stime-1} (a_0 - a_t)^\trans \x_t,
\end{equation}
then bounds the three terms separately. The
first sum is clearly bounded above by $\narms$.
We next work on bounding the third sum.
Let $s=\stime-1$.
\begin{align}
\left| (a_0 - \aemp{s})^\trans\,\, \vnpul_s \right|
    &\leq \sum_{j \in \arms} \rad(\aemp{s,j},\npul_{s,j})\, \npul_{s,j}
        \qquad\qquad\text{(by Lemma~\ref{lem:confrad-sum})} \nonumber \\
    &\leq \sqrt{\chernoffC \, \narms \asum} + \chernoffC \, \narms. \label{eq:vc.2} \\
\sum_{t=1}^{s} (a_0-a_t)^\trans\, \x_t
  &=
    a_0^\trans\, \vnpul_t - \sum_{t=1}^{s} a_t^\trans\, \x_t
   =
    (a_0 - \aemp{s})^\trans\, \vnpul_s.
 \nonumber \\
\left| \sum_{t=1}^{s} (a_0-a_t)^\trans\, \x_t  \right|
    &= \left| (a_0 - \aemp{s})^\trans\,\, \vnpul_s \right|
    \leq \sqrt{\chernoffC \, \narms \asum} + \chernoffC \, \narms. \nonumber
\end{align}

Finally we bound the middle sum in~\refeq{eq:vc.1}.
\begin{align}
      \left| \sum_{t=1}^{s} (b_t - a_0)^\trans \x_t \right|
  &\leq
      6 \sum_{t=1}^{s} \sum_{j \in \arms} \rad(a_{0,j}, \npul_{t,j}) \x_{t,j}
\nonumber \\
  &=
      6 \sum_{j \in \arms} \sum_{\ell=1}^{\npul_{s,j}} \rad(a_{0,j}, \ell)
\nonumber \\
  &=
      O \left( \sum_{j \in \arms}
            \sqrt{\chernoffC\, a_{0,j}\,\npul_{s,j}} + \chernoffC \log(\npul_{s,j})
%      \rad(a_{0,j},\npul_{s,j})\; \npul_{s,j} \;\log(\npul_{s,j}) \right)
        \right)
\nonumber \\
  & \leq
      O \left( \sqrt{\chernoffC \, \narms\, a_0^\trans\, \vnpul_s} + \chernoffC\, \narms\,            \log \horizon
        \right). \label{eq:vc.3}
\end{align}

We would like to replace the expression $a_0^\trans\, \vnpul_s$ on
the last line with the expression $\aemp{s}^\trans \,\vnpul_s = \asum$.
To do so, recall \eqref{eq:vc.2} and apply the following calculation:
\begin{align*}
a_0^\trans\, \vnpul_s
&\leq
    \aemp{s}^\trans \vnpul_s + \sqrt{\chernoffC \, \narms \asum}
         + \chernoffC \, \narms \\
&=
\asum + \sqrt{\chernoffC \, \narms \asum} + \chernoffC \, \narms \\
&\leq
\left( \sqrt{\asum} + \sqrt{\chernoffC \, \narms} \right)^2
\\
\sqrt{\chernoffC \, \narms a_0^\trans\, \vnpul_s}
   &\leq
\sqrt{\chernoffC \, \narms}
\left( \sqrt{\asum} + \sqrt{\chernoffC \, \narms} \right) =
\sqrt{\chernoffC \, \narms \asum} + \chernoffC \, \narms.
\end{align*}
Plugging this into \eqref{eq:vc.3}, we bound the middle sum in~\refeq{eq:vc.1} as
\begin{align}
      \left| \sum_{t=1}^{s} (b_t - a_0)^\trans \x_t \right|
 \leq
      O \left( \sqrt{\chernoffC \, \narms\asum} + \chernoffC\, \narms\,\log \horizon
        \right). \label{eq:vc.4}
\end{align}



Summing up the upper bounds for the three terms
on the right side of~\refeq{eq:vc.1}, we obtain~\refeq{eq:vector-conf}.
\end{proof}

\begin{corollary} \label{cor:error-terms}
In a clean execution of \pdbwk,
% if $\min \{\budg,\algrwd\} \geq \chernoffC \, \narms$, then
$$\left| \sum_{\narms<t<\stime} \rdif{t} \x_t \right| \leq
O \left( \sqrt{\chernoffC \, \narms  \algrwd} + \chernoffC \, \narms\, \log\horizon \right)$$
and
$$\left\| \sum_{\narms<t<\stime} \cdif{t} \x_t \right\|_{\infty} \leq
O \left( \sqrt{\chernoffC \, \narms  \budg} + \chernoffC \, \narms \, \log\horizon \right).$$
\end{corollary}
\begin{proof}
The first inequality is obtained by applying Lemma~\ref{lem:vector-conf}
with vector sequences $a_t = r_t$ and $b_t = u_t$. The second one is obtained
by applying the same lemma with vector sequences $a_t = (\sbv^\nrsc_i)^\trans\, C_t$ and
$b_t = \sbv^\nrsc_i\, L_t$, for each resource $i$.
\end{proof}




\begin{proofof}{Theorem~\ref{thm:pdbwk}}
If $\narms \geq \budg/\log(\nrsc\horizon)$, then the regret bound in Theorem~\ref{thm:pdbwk} is trivial. Therefore we can assume w.l.o.g. that $\narms \leq \budg/\log(\nrsc\horizon)$.
%Likewise, we can assume w.l.o.g. that $\narms \leq \LPOPT/\log(\nrsc\horizon)$.

Recall \eqref{eq:modulo-errors}. Since $\narms \leq \budg$, observe that
\[
2 \optlp \left( \sqrt{\frac{\ln \nrsc}{\budg}} + \frac{\narms+1}{\budg} \right)
=
O \left( \sqrt{\narms \log(\nrsc \narms \horizon)} \;
\frac{\optlp}{\sqrt{\budg}} \right).
\]
The term $m+1$ on the right side of~\eqref{eq:modulo-errors}
is bounded above by $m \log(\nrsc \narms \horizon)$.
Finally, using Corollary~\ref{cor:error-terms} we
% and recalling that $\chernoffC = \Theta(\log(\nrsc \narms \horizon))$,
see that the sum of the final two terms on the right side
of~\refeq{eq:modulo-errors} is bounded by
\begin{align*}
O \left( \sqrt{\chernoffC \, \narms} \left( \frac{\optlp}{\sqrt{\budg}} + \sqrt{\optlp}\right)
    + \chernoffC \, \narms \, \log\horizon   \right).
\end{align*}
The theorem follows by plugging in
    $\chernoffC = \Theta(\log(\nrsc \narms \horizon)) = O(\log(\nrsc \horizon)) $
(because $\narms\leq\budg\leq\horizon$).
\end{proofof}



%\begin{proofof}{Theorem~\ref{thm:pdbwk} and Theorem~\ref{thm:pdbwk-LP}}
%The first of these theorems asserts that
%\[
%\algrwd \geq \optrwd -
%O \left( \sqrt{\narms \log(\nrsc \narms \horizon)}
%\left( \frac{\optrwd}{\sqrt{\budg}} + \sqrt{\optrwd} + \sqrt{\narms \log(\nrsc \narms \horizon)}
%\right) \right).
%\]
%Denote the right-hand side by $f(\optrwd)$. The function
%$\max\{f(x),0\}$ is a non-decreasing function of $x$,
%so to establish both theorems we will prove that
%$\algrwd \geq f(\optlp) \geq f(\optrwd)$, where the latter
%inequality is an immediate consequence of the fact
%that $\optlp \geq \optrwd$ (Lemma~\ref{lem:lp-relax}).
%
%To prove $\algrwd \geq f(\optlp)$, we begin by recalling
%inequality~\refeq{eq:modulo-errors} and observing that
%\[
%2 \optlp \left( \sqrt{\frac{\ln \nrsc}{\budg}} + \frac{\narms+1}{\budg} \right)
%=
%O \left( \sqrt{\narms \log(\nrsc \narms \horizon)} \;
%\frac{\optlp}{\sqrt{\budg}} \right)
%\]
%by our assumption that $\narms \leq \budg$.
%The term $m+1$ on the right side of~\eqref{eq:modulo-errors}
%is bounded above by $m \log(\nrsc \narms \horizon)$.
%Finally, using Corollary~\ref{cor:error-terms} we
%% and recalling that $\chernoffC = \Theta(\log(\nrsc \narms \horizon))$,
%see that the sum of the final two terms on the right side
%of~\refeq{eq:modulo-errors} is bounded by
%$O \left( \sqrt{\chernoffC \, \narms} \left( \frac{\optlp}{\sqrt{\budg}} +
%\sqrt{\optlp} + \sqrt{\chernoffC \, \narms} \right) \right)$.
%The theorem follows by plugging in $\chernoffC = \Theta(\log(\nrsc
%\narms \horizon))$.
%\end{proofof}
%


==> BwK-probab.tex <==

\ascomment{!!! WE ARE NOT USING THIS FILE ANY MORE!!! (BwK-probab.tex)}

\xhdr{Additional notation.}
In addition to the averages $\empir{r}_p(x)$ and $\empir{c}_{i,p}(x)$, defined in Section~\ref{sec:Balance}, the analysis keeps track of several other quantities defined below.

For each arm $x$, consider all rounds in phases $q\leq p$ that are designated to arm $x$. Let $n_p(x)$ denote the number of times arm $x$ has been chosen in these rounds.
Let $\empirdtx{p}{x}=n_t(x)/p$ be the corresponding empirical probability of choosing $x$. Let 
    $\avedtx{p}{x}=\frac{1}{p}\sum_{q\leq p}\Dqx(x)$ 
be the average of probabilities for arm $x$ among the distributions chosen for these rounds.

Consider all rounds in phases $q\leq p$. There are $N = p|X|$ such rounds. 
Let 
    $\aveD_p = \tfrac{1}{N} \sum_{q\leq p,\, x\in X} \Dqx $ 
be the average distribution chosen by the algorithm in these rounds. Let 
    $\empir{r}_p = \tfrac{1}{N} \sum_{t=1}^N r_t$
be the average reward in these rounds.
Let
    $\empir{c}_{p,i} = \tfrac{1}{N} \sum_{t=1}^N c_{p,i}$
be the average consumption of resource each $i$ in these rounds.

\xhdr{High-probability events.} We consider several high-probability events which follow from applying Theorem~\ref{thm:conf-rad} to the various quantities defined above. All these events have the following common shape: for some $\nu, \empir{\nu} \in [0,1]$ and $N\in \N$, it holds that 
$|\nu - \empir{\nu}|
    \leq \rad(\empir{\nu},N)
    \leq 3\,\rad(\nu,N)$.
If this is the case, we will say that $\empir{\nu}$ is an \emph{$N$-strong estimator} for $\nu$.

\begin{lemma}\label{lm:high-prob-events}
For each phase $p$, arm $x$, and resource $i$, with probability $e^{-\Omega(\chernoffC)}$ it holds that:
\begin{itemize}
\item[(a)] $\empir{r}_p(x)$ is an $N_p(x)$-strong estimator for $r(x,\mu)$, and
$\empir{c}_{p,i}(x)$ is an $N_p(x)$-strong estimator for $c_i(x,\mu)$.

\item[(c)]  $\empirdtx{p}{x}$ is an $p$-strong estimator for $\avedtx{p}{x}$.

\item[(d)]  $\empir{r}_p$ is an $(p|X|)$-strong estimator for $r(\aveD_p,\, \mu)$,
and $\empir{c}_{p,i}$  is an $(p|X|)$-strong estimator for
 $c_i(\aveD_p,\, \mu)$.
\end{itemize}
\end{lemma}

A clean execution of the algorithm is one in which all events in Lemma~\ref{lm:high-prob-events} hold. In the rest of the analysis, we focus on a clean execution. 



